A spin-glass model for the loss surfaces of generative adversarial networks

We present a novel mathematical model that seeks to capture the key design feature of generative adversarial networks (GANs). Our model consists of two interacting spin glasses, and we conduct an extensive theoretical analysis of the complexity of the model's critical points using techniques from Random Matrix Theory. The result is insights into the loss surfaces of large GANs that build upon prior insights for simpler networks, but also reveal new structure unique to this setting.

==> oldstuff.tex <==


One consequence of this is that for $\sigma_z$ large enough, $H$ is well-approximated  by the first term and so \begin{align}
     |\det H| \approx \sigma_z^{N_D + N_G - 2} |\det\left(\sqrtsign{2^{p+q+1}(p+q)(p+q-1)(N_D + N_G - 2)}M_1 - (p+q)x_G2^{p+q}I\right)|
 \end{align}
 to which the results of \cite{auffinger2010random} immediately apply. We fix $N_D=300$ and try a few values of $N_G$. We also fix $p,q$ and we vary $\sigma_z$. The results are shown in Figures \ref{fig:complex_spectra} and \ref{fig:real_spectra}. Note:
 \begin{enumerate}[label=(\roman*)]
     \item The expected return towards to pure GOE statistics is seen for large enough $\sigma_z$.
     \item Large values of $N_G$ drag the statistics away from GOE, which is to be expected since the second term in (\ref{eq:H_rewritten}) has eigenvalue $0$ with multiplicity $N_G - 1$ and we indeed see an excess of mass around 0 in Figure \ref{fig:real_spectra} for large $N_G$.
     \item The similarity to Ginibre statistics in Figure \ref{fig:complex_spectra}.
 \end{enumerate}
\begin{comment}

By Lemma \ref{lemma:sc_conv_sc} we know that \begin{align}\label{eq:Fuv_def}
    \inf\{v\geq 0 ~|~ F(v, u) < y \} = \sqrtsign{y^{-1} + \frac{b_1^2}{2} - u^2}.
\end{align}
Consider a small change $\delta v$ in $v$ and small change in $\delta y$ in $y$. It follows that \begin{align}
    \frac{\delta y}{\delta v} \approx \frac{\delta F}{\delta v}
\end{align}
and so \begin{align}
    \frac{\partial F}{\partial v} = \left(\frac{\partial v}{\partial y}\right)^{-1} = -2y^2 v.
\end{align}
But \begin{align}
    y = \left(v^2 + u^2 - \frac{b_1^2}{2}\right)^{-1}
\end{align}
and so \begin{align}
    \frac{\partial F}{\partial v} = \frac{-2v}{v^2 + u^2 - \frac{b_1^2}{2}}\label{eq:dfdv_eq}.
\end{align}
We can solve (\ref{eq:dfdv_eq}) simply by anti-differentiation and matching (\ref{eq:Fuv_def}) as $v\rightarrow \infty$, giving \begin{align}
    F(v, u) = \left(v^2 + u^2 - \frac{b_1^2}{2}\right)^{-1}.
\end{align}
We can now directly solve \begin{align}
    &\kappa F(v, u)  + \frac{1-\kappa}{(u-\xi)^2 + v^2} < t^{-1}\notag\\
    \iff &\frac{v^4 + \left[u^2 - \frac{b_1^2}{2} + (u-\xi)^2 - \frac{b^2\kappa'(1+\rho)}{2}\right]v^2 + \frac{1}{2}\left[(u-\xi)^2(2u^2 - b_1^2) - b^2\kappa'\left(u^2 - \frac{b_1^2}{2} + \rho(u-\xi)^2\right)\right]}{\left(v^2 + u^2 - \frac{b_1^2}{2}\right)\left( (u-\xi)^2 + v^2\right)} > 0\label{eq:vt_quartic}
\end{align}
where the second line follows from a line of simple manipulation. Suppose first that the numerator in (\ref{eq:vt_quartic}) has no real roots for $v^2$, then the numerator is positive for all $v \geq 0$ and so \begin{align}
    v_t(u) = \sqrtsign{\max\left\{\frac{b_1^2}{2} - u^2, 0\right\}} = \mathbbm{1}_{|u| < \frac{b_1}{\sqrtsign{2}}}\sqrtsign{\frac{b_1^2}{2} - u^2}.
\end{align}
Now suppose that (\ref{eq:vt_quartic}) has two real roots $r_1 < r_2$ for $v^2$. If $u^2 > \frac{b_1^2}{2}$ then the denominator in (\ref{eq:vt_quartic}) positive for all $v\geq 0$ and so $v_t(u) = 0$ if both roots are the same sign and otherwise  $v_t(u) = \sqrtsign{r_2}$. Finally, if $u^2 < \frac{b_1^2}{2}$, then there are three cases: \begin{enumerate}
    \item $\frac{b_1^2}{2} - u^2  < r_1 ~ \implies ~ v_t(u) = \sqrtsign{\frac{b_1^2}{2} - u^2},$
    \item $r_1 < \frac{b_1^2}{2} - u^2  < r_2 ~ \implies ~ v_t(u) = \sqrtsign{\max\{0, r_1\}},$
    \item $ 0 < r_2 < \frac{b_1^2}{2} - u^2 ~ \implies ~ v_t(u) = 0.$
\end{enumerate}
Note that these are the only possibilities since other arrangements leave $v_t(u)$ undefined, which is impossible by \cite{biane1997free}.

 Moreover (\ref{eq:psi_t_expr}) can be replaced by \cite{biane1997free} \begin{align}\label{eq:psi_real}
    \psi_t(u) = \Re H_t(u + iv_t(u))
\end{align} where \begin{align}
    H_t(z) = z + t G_{\mu_1}(z) = z + \frac{b^2}{2}G_{\mu_1}(z)
\end{align}
and $G_{\mu_1}$ is the Stieljes transform of $\mu_1$ so \begin{align}\label{eq:mu1_stieljes}
    G_{\mu_1}(z) = (1-\kappa)(z-\xi)^{-1} + \frac{\kappa}{b_1^2} \left(z - \sqrtsign{z^2 - 2b_1^2}\right).
\end{align}
This procedure (\ref{eq:psi_real} - \ref{eq:mu1_stieljes}) is much more numerically straightforward than (\ref{eq:psi_t_expr}). Figure \ref{fig:free_conv_numerical_eg} shows an example solve for some arbitrarily chosen parameters. We note that it is still not quite right, in particular there seem to be difficulties towards the edges of the intervals constituting the support, which is presumably due to the non-unifrom resolution introduced by $\psi_t$ in the parametric form (\ref{eq:density_v_psi}). More nuanced numerical treatment required.

\begin{figure}
    \centering
    \includegraphics{free_conv_numerics_eg.pdf}
    \caption{Example of empirical eigenvalue spectrum (histogram in blue) and theoretical prediction of limiting density for $\kappa=0.7, \xi=2, b=b_1=1$.}
    \label{fig:free_conv_numerical_eg}
\end{figure}

However, since solving for $v_t(u)$ is analytically simple (if ugly), requiring only the solution of a quadratic (\ref{eq:phi_quadratic}), then if it is possible to apply a suitable transformation to the integral (\ref{eq:psi_t_expr}) then it may become tractable. Let $f_{C}(x; x_0, \gamma)$ be the density of the Cauchy distribution, so \begin{align}
   f_{C}(x; x_0, \gamma) = \frac{1}{\pi\gamma} \left(\frac{\gamma^2}{\gamma^2 + (x-x_0)^2}\right).
\end{align}
Notice that \begin{align}
 \frac{\partial}{\partial x} \log f_{C}(x; x_0, \gamma) = \frac{2(x-x_0)}{\gamma^2 + (x-x_0)^2}
\end{align}
and so \begin{align}
    \frac{\kappa}{b_1^2\pi} \int_{-\sqrtsign{2}b_1}^{\sqrtsign{2}b_1} \frac{(u-x)\sqrtsign{2b_1^2 - x^2}}{(u-x)^2 + v_t(u)^2}dx = -\frac{1}{2}\frac{1}{b_1^2\pi} \int_{-\sqrtsign{2}b_1}^{\sqrtsign{2}b_1}\sqrtsign{2b_1^2 - x^2} \frac{\partial}{\partial x} \log f_{C}(x; u, v_t(u)) dx.
\end{align}
\end{comment}
\begin{comment}
\section{Large deviations}
Supposing that we could progress with the previous section, to obtain the Hessian index prescription results as in \cite{baskerville2020loss}, we would ideally have an LDP for (up-to constant in front of the matrices) \begin{align}
  M \equiv  M_1 + \left(\begin{array}{cc}
         M_2 &0  \\
         0 & 0
    \end{array}\right)
\end{align}
    for GOE $M_1, M_2$. I have struggled to find any literature approaching such a thing. Note further that (\ref{eq:H_rewritten}) is not simply a characteristic polynomial of  $M$.
    
    \section{Spectrum of the block GOE matrix}
    As in the previous section, some results relating to the spectrum of   M \begin{align}
  M \equiv  M_1 + \left(\begin{array}{cc}
         M_2 &0  \\
         0 & 0
    \end{array}\right)
\end{align}
would be most useful. If we could obtain the equilibrium measure, then we should be able to get the order of magnitude for the complexity. Note again that (\ref{eq:H_rewritten}) is not simply a characteristic polynomial of  $M$ so even having the equilibrium measure for $M$ wouldn't necessarily solve the problem straight away.
\begin{comment}
 \begin{figure}
     \centering
     \includegraphics[width=\linewidth]{GAN_spectra_scatter_30_samples.pdf}
     \caption{Scatter plot in complex plane of eigenvalues of the stochastic matrix in (\ref{eq:H_first}). $N_D=300$, $p,q=5$ throughout, but $N_G$ and $\sigma_z$ are varied. Plots are produced by combining 30 sample matrices and the spectra are normalised by $\sqrtsign{N_D + N_G}$.}
     \label{fig:complex_spectra}
 \end{figure}
 
 \begin{figure}
     \centering
     \includegraphics[width=\linewidth]{GAN_spectra_sym_30_samples.pdf}
     \caption{Histogram and KDE plot of eigenvalues of the stochastic matrix in (\ref{eq:H_rewritten}). $N_D=300$, $p,q=5$ throughout, but $N_G$ and $\sigma_z$ are varied. Plots are produced by combining 30 sample matrices and the spectra are normalised by $\sqrtsign{N_D + N_G}$. The red lines show the semi-circle laws with the same support as the empirical distributions.}
     \label{fig:real_spectra}
 \end{figure}
 \end{comment}
 \end{comment}
 
 
 
 
 
  
 
\begin{comment}
   \section{Supersymmetric approach} 
 \subsection{No Hessian index prescription} 
We will express the absolute value of the determinant as a supersymmetric integral as in \cite{baskerville2020loss}. There are numerous routes through the problem from that point including \begin{enumerate}
    \item follow \cite{baskerville2020loss,nock2017characteristic} as closely as possible;
    \item follow \cite{guhr1990isospin} directly.
\end{enumerate}
 Both of these approaches (and variants thereof) result in integrals in intractable saddle point calculations, soluble only by numerical methods but this is unsatisfactory since the determination of the branch structure in the $x_D, x_G$ planes is intractable. \cite{guhr1990isospin} obtains simple single-variable quadratic equations for a fixed number of intermediate integration variables allowing for analytic solution and easy analysis of the branch structure. The central issue is this: if we proceed directly as \cite{guhr1990isospin} and perform the Hubbard-Stratanovich transformation in super-space, our expression lacks a certain symmetry that is presents in the calculations of \cite{guhr1990isospin} which turns out to be critical in making the saddle point calculations analytically tractable. This asymmetry is due to the structural asymmetry in (\ref{eq:H_rewritten}, namely between the upper-left and bottom-right blocks. We here propose the remedy this problem by introducing extra terms in (\ref{eq:H_rewritten}) that provide just enough symmetry to allow for an application of the method in \cite{guhr1990isospin}. We will then recover the desired quantity by taking an appropriate limit. Consider the matrix \begin{align}
     \sqrtsign{2N}bM - xI + \sqrtsign{2\kappa N} b_1 \left(\begin{array}{cc}
     M_1 & 0 \\ 0 & 0\end{array}\right) - x_1\left(\begin{array}{cc}
     I & 0 \\ 0 & 0\end{array}\right) + \sqrtsign{2\kappa' N} b_2 \left(\begin{array}{cc}
     0 & 0 \\ 0 & M_2\end{array}\right) - x_2\left(\begin{array}{cc}
     0 & 0 \\ 0 & I\end{array}\right) \label{eq:susy_surrogate_N}
 \end{align}
 where $b_2, x, x_1, x_2\in\mathbb{R}$ are parameters we are free to tune to recover the desired quantity and $M\sim GOE^N, M_1\sim GOE^{\kappa N}, M_2\sim GOE^{\kappa' N}$. We factor out the $\sqrtsign{2N}$ and so study the random matrix \begin{align}\label{eq:symmetric-block-matrix}
     \mathcal{M} \overset{d}{=} bM -xI+ \sqrtsign{\kappa}b_1 \left(\begin{array}{cc}
     M_1 & 0 \\ 0 & 0\end{array}\right) - x_1\left(\begin{array}{cc}
     I & 0 \\ 0 & 0\end{array}\right) + \sqrtsign{\kappa'} b_2 \left(\begin{array}{cc}
     0 & 0 \\ 0 & M_2\end{array}\right) - x_2\left(\begin{array}{cc}
     0 & 0 \\ 0 & I\end{array}\right)
 \end{align}
 where $\sqrtsign{2N}$ factors have been absorbed into the free parameters. As in \cite{baskerville2020loss} we use \begin{align}\label{eq:delta-def}
     |\det \mathcal{M}| = \lim_{\epsilon\searrow 0} \frac{\det(\mathcal{M} - i\epsilon)\det(\mathcal{M} + i\epsilon)}{\sqrtsign{{\det(\mathcal{M} - i\epsilon)}}\sqrtsign{\det(\mathcal{M} + i\epsilon)}} \equiv \lim_{\epsilon\searrow 0}\Delta_{\epsilon}
 \end{align}
 and then, moving to the supersymmetric representation \begin{align}
     \Delta_{\epsilon} = K_N^{(1)} \int&\prod_{t=1}^2 d\vec{x}_1[t]d\vec{x}_2[t] d\zeta_1[t]d \zeta_1^*[t]d\zeta_2[t] d\zeta_2^*[t]\notag\\
     &\exp\left\{-ib\Tr MA - ib_1\sqrtsign{\kappa}\Tr M_1A[1] - ib_2\sqrtsign{\kappa'}\Tr M_2A[2] + ix\Tr{A} + ix_1 \Tr{A[1]} + ix_2\Tr{A[2]}\right\} \label{eq:no_hessian_k_delta}
 \end{align}
 where \begin{align}
     A = \vec{x}_1\vec{x}_1^T + \vec{x}_2\vec{x}_2^T + \zeta_1\zeta_1^{\dagger} + \zeta_2\zeta_2^{\dagger}
 \end{align}
 and $A[1], A[2]$ are defined similarly. Note that we have dropped the $\epsilon$ terms. These terms play an important role in determining branch structure at later stages in the calculation as in \cite{baskerville2020loss} but it is only their sign that matters. To proceed rigorously, we must retain the $\epsilon$ terms and introduce explicit angular integrals arising from parametrisations the graded group $SU(2/4)$. We choose instead to proceed formally by dropping the $\epsilon$ terms and reintroducing them at the end. It is intuitive that this approach will yield the correct result.
Let us use the shorthand  \begin{equation}
     \mathcal{D} \Psi = \prod_{t=1}^2\mathcal{D}\Psi[t] \prod_{t=1}^2 d\vec{x}_1[t]d\vec{x}_2[t] d\zeta_1[t]d \zeta_1^*[t]d\zeta_2[t] d\zeta_2^*[t].
 \end{equation}
 As desired, performing the matrix averages is now simple, giving \begin{align}
     \mathbb{E}\Delta_{\epsilon} = K_N^{(1)} \int\mathcal{D}\Psi
     \exp\left\{-\frac{b^2}{N}\trg Q^2 - -\frac{b_1^2}{N}\trg Q[1]^2  -\frac{b_2^2}{N}\trg Q[2]^2 + ix\trg{Q} + ix_1 \trg{Q[1]} + ix_2\trg{Q[2]}\right\} \label{eq:no_hessian_k_expect_delta}
 \end{align}
 where the $6\times 6$ matrix $Q$ is given by \begin{align}
     Q = \left(\begin{array}{cccccc}
     \vec{x}_1^T\vec{x}_1 &  \vec{x}_1^T\vec{x}_2 &  \vec{x}_1^T\zeta_1 &  \vec{x}_1^T\zeta_1^* &  \vec{x}_1^T\zeta_2 &  \vec{x}_1^T\zeta_2^*\\
      \vec{x}_2^T\vec{x}_1 &  \vec{x}_2^T\vec{x}_2 &  \vec{x}_2^T\zeta_1 &  \vec{x}_2^T\zeta_1^* &  \vec{x}_2^T\zeta_2 &  \vec{x}_2^T\zeta_2^*\\
        \zeta_1^T\vec{x}_1 &   \zeta_1^T\vec{x}_2 &   \zeta_1^T\zeta_1 &   \zeta_1^T\zeta_1^* &   \zeta_1^T\zeta_2 &  \zeta_1^T\zeta_2^*\\
        \zeta_1^{\dagger}\vec{x}_1 &   \zeta_1^{\dagger}\vec{x}_2 &   \zeta_1^{\dagger}\zeta_1 &   \zeta_1^{\dagger}\zeta_1^* &   \zeta_1^{\dagger}\zeta_2 &  \zeta_1^{\dagger}\zeta_2^*\\
        \zeta_2^T\vec{x}_1 &   \zeta_2^T\vec{x}_2 &   \zeta_2^T\zeta_1 &   \zeta_2^T\zeta_1^* &   \zeta_2^T\zeta_2 &  \zeta_2^T\zeta_2^*\\
        \zeta_2^{\dagger}\vec{x}_1 &   \zeta_2^{\dagger}\vec{x}_2 &   \zeta_2^{\dagger}\zeta_1 &   \zeta_2^{\dagger}\zeta_1^* &   \zeta_2^{\dagger}\zeta_2 &  \zeta_2^{\dagger}\zeta_2^*
     \end{array}\right)
 \end{align}
 and  $Q[1], Q[2]$ are given similarly. Note that $Q = Q[1] + Q[2]$. We now follow \cite{guhr1990isospin} in performing 3 Hubbard-Stratanovich transformations \begin{align}
     \mathbb{E}\Delta_{\epsilon} = &K_N^{(1)}\int  d\sigma\prod_{t=1}^2\mathcal{D}\Psi[t]d\sigma[t]\notag\\\ &\exp\left\{-\frac{N}{4b^2}\trg \sigma^2 - -\frac{N}{4b_1^2}\trg \sigma[1]^2  -\frac{N}{4b_2^2}\trg \sigma[2]^2 +i\trg\left(\sigma[1] + \sigma + x + x_1\right)Q[1] + +i\trg\left(\sigma[2] + \sigma + x + x_2\right)Q[2]\right\}\notag\\
     = &K_N^{(1)}\int  d\sigma\prod_{t=1}^2\mathcal{D}\Psi[t]d\sigma[t]\notag\\\ &\exp\left\{-\frac{N}{4b^2}\trg \sigma^2 - -\frac{N}{4b_1^2}\trg \sigma[1]^2  -\frac{N}{4b_2^2}\trg \sigma[2]^2 +i\Psi[1]^T\left(\sigma[1] + \sigma + x + x_1\right)\Psi[1] +i\Psi[2]^T\left(\sigma[2] + \sigma + x + x_2\right)\Psi[2]\right\}
 \end{align}
 where the $\sigma, \sigma[1], \sigma[2]$ integrals are performed over all supermatrices with the same structure as $Q$ (and so as $Q[1], Q[2]$). Note the high level of structural symmetry in the preceding expression and that this symmetry would be lacking were it not for the $\sigma[2]$ and $x_2$ terms. The $\sigma$ matrices are therefore Hermitian 2/4 supermatrices. We can then finally compute the $\Psi$ integrals to give \begin{align}
      \mathbb{E}\Delta_{\epsilon} = K_N^{(1)}\int & d\sigma\prod_{t=1}^2\mathcal{D}\Psi[t]d\sigma[t] \exp\left\{-\frac{N}{4b^2}\trg \sigma^2 - -\frac{N}{4b_1^2}\trg \sigma[1]^2  -\frac{N}{4b_2^2}\trg \sigma[2]^2\right\}\notag\\
      &\left(\detg\left(\sigma[1] + \sigma + x + x_1\right)\right)^{-\frac{\kappa N}{2}}\left(\detg\left(\sigma[2] + \sigma + x + x_1\right)\right)^{-\frac{\kappa' N}{2}}\notag\\
      = K_N^{(1)}\int & d\sigma\prod_{t=1}^2\mathcal{D}\Psi[t]d\sigma[t]\notag\\
      &\exp\Bigg\{-\frac{N}{4b^2}\trg \sigma^2  -\frac{N}{4b_1^2}\trg \left(\sigma[1] - \sigma\right)^2-\frac{N}{4b_2^2}\trg \left(\sigma[2] - \sigma\right)^2\notag\\
      &- \frac{\kappa N}{2} \trg\log\left( \sigma[1] + x + x_1\right)- \frac{\kappa' N}{2} \trg\log\left( \sigma[2] + x + x_2\right)\Bigg\}\label{eq:symmetric_sigma_rep}
 \end{align}
 where on the second line we have made simple change of variables in $\sigma[1],\sigma[2]$.
 As in \cite{guhr1990isospin} we will now perform the saddle point approximation \emph{on the} $\sigma$ \emph{manifolds} (the so-called `coset method'). Varying each of the $ \sigma[1], \sigma[2], \sigma$ respectively gives the following variational equations at a saddle point \begin{align}
     \frac{1}{2b_1^2} (\sigma - \sigma[1]) - \frac{\kappa}{2}\left(\sigma[1] + x + x_1\right)^{-1} &= 0\label{eq:coset1}\\
  \frac{1}{2b_2^2} (\sigma - \sigma[2]) - \frac{\kappa'}{2}\left(\sigma[2] + x + x_2\right)^{-1} &= 0\label{eq:coset2}\\
   \frac{1}{2b^2} \sigma- \frac{1}{2b_1^2}\left(\sigma - \sigma[1]\right) - \frac{1}{2b_2^2}\left(\sigma - \sigma[2]\right)&= 0.\label{eq:coset3}
 \end{align}
 Note that we can diagonalise $\sigma$ and absorb any diagonalising $SU(2/4)$ matrix terms into $\sigma[1], \sigma[2]$. We therefore take $\sigma$ diagonal hereafter. We propose the ansatz $\sigma[1] = 
\eta\sigma[2]$ for some $\eta\in\mathbb{C}$. It follows immediately from (\ref{eq:coset3}) that $\sigma[1], \sigma[2]$ are diagonal also. Say $\sigma[2] = \text{diag}(\sigma_1, \ldots, \sigma_6)$ Further, (\ref{eq:coset1}-\ref{eq:coset2}) each give a quadratic equation for the $\sigma_i$ and so requiring the equations to agree gives (matching the quadratic terms) \begin{equation}\label{eq:eta_quadratic}
    \frac{1}{\kappa b_1^2} \eta \left(\eta b_2^2 b^{-2} + \eta - 1\right) =  \frac{1}{\kappa' b_2^2} \eta \left( b_2^2 (b^{-2} + b_1^{-2}) - \eta b_2^2 B_1^{-2}\right)
\end{equation}
and (matching linear terms) \begin{equation}\label{eq:eta_linear}
    \frac{1}{\kappa b_1^2} (x_1 + x) (\eta b_2^2b^{-2} + \eta - 1) = \frac{1}{\kappa' b_2^2}(x_2 + x) \left(b_2^2(b^{-2} + b_1^{-2}) - \eta b_s^2b_1^{-2}\right).
\end{equation}
 Solving (\ref{eq:eta_quadratic}) gives a positive and negative solution, so we take the positive solution for the sake of definiteness. Having fixed $\eta$ (\ref{eq:eta_linear}) gives a relationship between $x, x_1, x_2$. The solutions are \begin{align}
     \eta &= \frac{1-\rho + \left((\rho-1)^2 + 4\rho\left( 1 + b_1^{2}b^{-2} \right)\left( 1 + b_2^2b^{-2}\right) \right)^{1/2}}{2\left(b_2^2b^{-2} +1 \right)},\\
     x + x_2 &= \frac{\rho^{-1}\left(\eta b_2^2b^{-2} + \eta - 1\right)}{\beta^2 +1 - \eta} ( x + x_1)
 \end{align} where we have defined \begin{align}
   \rho = \frac{\kappa}{\kappa'}, ~~~ \beta = \frac{b_1}{b}.
 \end{align} Ultimately, we are interested in the limit $b_2\rightarrow 0$ and so we record the solutions to (\ref{eq:eta_quadratic}-\ref{eq:eta_linear}) in that limit:\begin{align}
     \eta &= \frac{1}{2}\left( 1 - \rho + \sqrtsign{(\rho -1)^2 + 4\rho(\beta^2 + 1)}\right)\\
     x + x_2 &= \underbrace{\frac{\rho^{-1}(\eta - 1)}{\beta^2 + 1 - \eta}}_{{\equiv\varphi}}(x + x_1)\label{eq:x2x1_rel} .
 \end{align}

Solving (\ref{eq:coset3}) simply gives \begin{align}
    \sigma = \frac{\eta b_2^2b_1^{-2} + 1}{b_2^2(b^{-2} + b_1^{-2}) + 1}\sigma[2]
\end{align}
which in the $b_2\rightarrow 0$ reduces to $\sigma = \sigma_2$. Solving (\ref{eq:coset1}) for $\sigma_1,\ldots, \sigma_6$ gives (in the $b_2\rightarrow 0$ limit) \begin{align}\label{eq:sigma_sol}
    \sigma_i = \frac{1}{2\eta} \left[ -X_{\epsilon}^{(-)^i} + \left( (X_{\epsilon}^{(-)^i})^2 - 2\kappa b_1^2 \eta (\eta - 1)^{-1}\right)^{1/2}\right]
\end{align}
where we have defined \begin{equation}\label{eq:Xeps}
    X_{\epsilon}^{(\pm)} = x + x_1 \pm i\epsilon.
\end{equation}
Note that we have reintroduced the $\epsilon$ terms. A little thought and comparison with (\ref{eq:delta-def}) convinces one that this is the correct expression with the correct signs on the $\epsilon$ terms. Note also the familiarity of the expression (\ref{eq:sigma_sol}) and the natural radius parameter is $r = \sqrtsign{2\kappa b_1^2 \eta (\eta - 1)^{-1}}.$

The condition must be enforced along with \begin{align}
    x' &= x + x_2, \label{eq:xcond1}\\
    x' + x_1' &= x + x_1,\label{eq:xcond2}
\end{align} giving the constraint\begin{equation}
    x' = \frac{\varphi}{1 - \varphi} x_1'
\end{equation} which we enforce with a Fourier delta function representation \begin{align}
    \delta(x - \varphi(1-\varphi)^{-1}) = \int_{\mathbb{R}}d\xi \exp\left\{2\pi i\xi \left(x - \frac{\varphi}{1-\varphi}\right)\right\}.\label{eq:fourier_delta}
\end{align}
Now define the exponent function \begin{align}
    \L  &= \frac{1}{4b^2} \trg\sigma^2 + \frac{1}{4b_1^2} \trg(\sigma - \sigma[1])^2 + \frac{1}{4b_2^2} \trg(\sigma - \sigma[2])^2 + \frac{\kappa}{2} \trg\log\left(\sigma[1] + x + x_1\right) + \frac{\kappa'}{2}\trg\log\left(\sigma[2] + x + x_2\right).
\end{align}
We need to sub-in the conditions (\ref{eq:xcond1}-\ref{eq:xcond2}) and and evaluate in the $b_2\rightarrow 0$ limit. Firstly \begin{align}
    \sigma - \sigma[2] &=  \frac{\eta b_2^2b_1^{-2} - b_2^2(b^{-2} + b_1^{-2})}{  b_2^2(b^{-2} + b_1^{-2}) + 1}\sigma[2]\notag\\
    \implies \frac{1}{b_2^2} (\sigma - \sigma[2])^2 &\propto b_2^2 \rightarrow  0
\end{align}
and \begin{align}
    \sigma - \sigma[1] \rightarrow (\eta - 1)\sigma[2]
\end{align}
so we have the exponent function \begin{align}
    \L = &\left(\frac{1}{4b^2} + \frac{1}{4b_1^2}(\eta - 1)^2\right) \trg \sigma[2]^2 + \frac{\kappa}{2} \trg\log\left( \eta\sigma[2] + x' + x_1'\right) + \frac{\kappa'}{2} \trg\log\left(\sigma[2] + x'\right)\notag\\
    =&\left(\frac{1}{4b^2} + \frac{1}{4b_1^2}(\eta - 1)^2\right) \left(\sigma_1^2 + \sigma_2^2 - \sigma_3^2 -\ldots - \sigma_6^2\right)+  \frac{\kappa}{2} \trg\log\left( \eta\sigma[2] + x' + x_1'\right) + \frac{\kappa'}{2} \trg\log\left(\sigma[2] + x'\right).
\end{align}

We now need to evaluate $\L$ using (\ref{eq:sigma_sol}) which gives \begin{align}
    \L\Bigg|_{\text{saddle}} = &\frac{1}{4\eta}\sum_{s\in \{\pm\}} \left(b^{-2} + b_1^{-2}(\eta-1)^2\right)\left[ -\frac{1}{2\eta} (X_{\epsilon}^s)^2 + \frac{1}{2\eta} X_{\epsilon}^s \left((X_{\epsilon}^s)^2 - r^2\right)^{1/2} + \frac{\kappa}{2}b_1^2(\eta - 1)^{-1}\right]\notag\\
    & -\frac{1}{2}\sum_{s\in\{\pm\}}\left\{\kappa \log\left(\frac{1}{2}\left[-X_{\epsilon}^s + \left( (X_{\epsilon}^s)^2 - r^2\right)^{1/2}\right] + X_{\epsilon}^s\right) + \kappa'\log\left(\frac{1}{2}\left[-X_{\epsilon}^s + \left( (X_{\epsilon}^s)^2 - r^2\right)^{1/2}\right] + x' + is\epsilon\right)\right\}
\end{align}
where, note, due to (\ref{eq:Xeps}) and (\ref{eq:xcond2}) we have \begin{align}
    X_{\epsilon}^{\pm} = x' + x_1' \pm i\epsilon.
\end{align}

We wish to integrate over $ L^{(D)} \in (-\infty, \sqrtsign{N} u_D)$ and $L^{(G)} \in (-\infty, \sqrtsign{N} u_G)$.  $L^{(D)}$ has unit variance and $ L^{(G)}$ has variance $2^{p+q}$.  Recall that\footnote{Factors $(2N)^{-1/2}$ come from the absorbed factor of $\sqrtsign{2N}$ between (\ref{eq:susy_surrogate_N}) and (\ref{eq:symmetric-block-matrix}).} $x_1' = -px_D (2N)^{-1/2}$ and $x' = \sigma_z (p+q) 2^{p+q} x_G (2N)^{-1/2}$ and so we need to integrate against the measures \begin{align}
    \sqrtsign{\frac{N}{2\pi s^2}}e^{-\frac{N}{2s^2}(x')^2}dx',~~~ \sqrtsign{\frac{N}{2\pi s_1^2}} e^{ -\frac{N}{2s_1^2} (x_1')^2}dx_1'
\end{align}
over the set \begin{align}
    B' = \left\{(x', x_1')\in\mathbb{R}^2 ~:~ x'\leq \frac{1}{\sqrtsign{2}}(p+q)2^{p+q} u_G, ~~ x_1' \geq -(p+q)^{-1} 2^{-(p+q)}p x' - \frac{p}{\sqrtsign{2}}u_D\right\}.
\end{align}
where \begin{align}
    s^2 = \frac{1}{2}\sigma_z^2(p+q)^2 2^{3(p+q)}, ~~~ s_1^2 = \frac{p^2}{2}.
\end{align}
We now change variables $y_1 = x' + x_1'$ and $y_2 = x'$ and so \begin{align}
    \iint_{B} dy_1dy_2 \int_{\mathbb{R}} d\xi e^{2\pi i\xi\left(x - \frac{\varphi}{1-\varphi}\right)} e^{-\frac{N}{2s^2}y_2^2} e^{-\frac{N}{2s_1^2}(y_1 - y_2)^2} e^{- N\L(y_1, y_2)}
\end{align}
where \begin{align}
    \L(y_1, y_2) = &\frac{1}{4\eta} \sum_{s\in\{\pm\}} \left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)\left(-\frac{1}{2\eta} (y_1 + is\epsilon)^2 + \frac{1}{2\eta} (y_1 + is\epsilon)\left((y_1 + is\epsilon)^2 - r^2\right)^{1/2} + \frac{r^2}{4\eta}\right)\notag\\
    & - \frac{1}{2}\sum_{s\in\{\pm\}}\Bigg\{\kappa\log\frac{1}{2}\left[(y_1 + is\epsilon) + \left((y_1 + is\epsilon)^2 - r^2\right)^{1/2}\right] \notag\\ &+\kappa'\log\frac{1}{2}\left[\frac{1}{\eta}\left(-(y_1 + is\epsilon) + \left((y_1 + is\epsilon)^2 - r^2\right)^{1/2}\right) + 2(y_2 + is\epsilon)\right] \Bigg\}
\end{align}
and \begin{align}
    B = \left\{(y_1, y_2)\in\mathbb{R}^2 ~:~ y_2 \leq \frac{1}{\sqrtsign{2}}(p+q)2^{p+q}u_G, ~ y_1\geq \left(1 - \frac{p}{(p+q) 2^{p+q}}\right)y_2 - \frac{pu_D}{\sqrtsign{2}}\right\}
\end{align}
Recalling the asymptotic analysis in \cite{baskerville2020loss}, $y_1=r$ is the dividing line of interest with regard the branch structure in the variables $y_1$. Indeed, for $|y_1| > r$ (implicitly taking $\epsilon\searrow 0$) (c.f. branch cuts in \cite{baskerville2020loss}) \begin{align}
    \L(y_1, y_2)= &\frac{1}{2\eta}  \left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)\left(-\frac{1}{2\eta} y_1^2 +  \frac{1}{2\eta} |y_1|\sqrtsign{y_1^2 - r^2} + \frac{r^2}{4\eta}\right)\notag\\
    & -\kappa\log\frac{1}{2}\left[y_1 + \text{sgn}(y_1)\sqrtsign{y_1^2 - r^2}\right]-\kappa'\log\frac{1}{2}\left[\frac{1}{\eta}\left(-y_1 + \text{sgn}(y_1)\sqrtsign{y_1^2- r^2}\right) + 2y_2 \right] \label{eq:l_saddle_outbulk}
\end{align}
and for $|y_1| < r$ \begin{align}
        \L(y_1, y_2)= &\frac{1}{2\eta} \left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)\left(-\frac{1}{2\eta} y_1^2 +\frac{r^2}{4\eta}\right)\notag\\
    & -\frac{\kappa}{2}\log\frac{r^2}{4}-\frac{\kappa'}{2}\sum_{s\in\{\pm\}}\log\frac{1}{2}\left[\frac{1}{\eta}\left(-y_1 + is\sqrtsign{r^2- y_1^2}\right) + 2y_2 \right] \notag\\
  = &\frac{1}{2\eta} \left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)\left(-\frac{1}{2\eta} y_1^2 +\frac{r^2}{4\eta}\right)\notag\\
    & -\frac{\kappa}{2}\log\frac{r^2}{4}-\frac{\kappa'}{2}\log\frac{1}{4}\left(r^2\eta^{-2} + 4y_2^2 - 4y_1y_2\eta^{-1}\right).\label{eq:l_saddle_inbulk}
\end{align}

Writing \begin{align}
    \iint_{B} dy_1dy_2 \int_{\mathbb{R}} d\xi e^{2\pi i\xi\left(x - \frac{\varphi}{1-\varphi}\right)} e^{-\frac{N}{2s^2}y_2^2} e^{-\frac{N}{2s_1^2}(y_1 - y_2)^2} e^{- N\L(y_1, y_2)} =
    \iint_{B} dy_1dy_2 \int_{\mathbb{R}} d\xi e^{2\pi i\xi\left(x - \frac{\varphi}{1-\varphi}\right)}e^{-N\Phi}
\end{align}
we have for $|y_1| > r$\begin{align}
    \Phi(y_1, y_2) &= \frac{y_2^2}{2s^2} + \frac{(y_2 - y_1)^2}{p^2} + \frac{1}{2\eta}  \left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)\left(-\frac{1}{2\eta} y_1^2 +  \frac{1}{2\eta} |y_1|\sqrtsign{y_1^2 - r^2} + \frac{r^2}{4\eta}\right)\notag\\
    & -\kappa\log\frac{1}{2}\left[y_1 + \text{sgn}(y_1)\sqrtsign{y_1^2 - r^2}\right]-\kappa'\log\frac{1}{2}\left[\frac{1}{\eta}\left(-y_1 + \text{sgn}(y_1)\sqrtsign{y_1^2- r^2}\right) + 2y_2 \right]\label{eq:phi_outside}
\end{align} and for $|y_1| < r$ \begin{align}
    \Phi(y_1, y_2) &= \frac{y_2^2}{2s^2} + \frac{(y_2 - y_1)^2}{p^2} + \frac{1}{2\eta} \left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)\left(-\frac{1}{2\eta} y_1^2 +\frac{r^2}{4\eta}\right)\notag\\
    & -\frac{\kappa}{2}\log\frac{r^2}{4}-\frac{\kappa'}{2}\log\frac{1}{4}\left(r^2\eta^{-2} + 4y_2^2 - 4y_1y_2\eta^{-1}\right)\label{eq:phi_inside}
\end{align}
It is apparent from inspecting these previous two expressions results that $\Phi$ is bounded below on all of $\mathbb{R}^2$. We may have to worry slightly about singularities of the logarithms in the $|y_1|>r$ expression, but the log term for $|y_1|<r$ has strictly positive argument for $|y_1|<r$. Numerics seems to show that $\Phi$ attains its minimum on $\partial B$ in general. Say $\partial B = T_h \cup T_d$ where \begin{align}
    T_h &= \{(y_1, y_2)\in\mathbb{R}^2 ~|~ y_2 = \frac{p+q}{\sqrtsign{2}}2^{p+q} u_G\}\\
      T_d &= \left\{(y_1, y_2)\in\mathbb{R}^2 ~|~ y_1 = \left( 1 - \frac{p}{(p+q)2^{p+q}}\right)y_2 - \frac{p u_D}{\sqrtsign{2}}\right\}.
\end{align} Below some critical values of $u_G, u_D$ it appears that the minimum is attained on $T_h\cap T_d$ (a singleton set, of course). Above that criticality, it appears that the minimum is attained at some fixed point on $T_d$. This is strongly reminiscent of \cite{baskerville2020loss}.


We can illuminate some different cases with heuristics. We first need to record the intersection of $y_2 = y_1$ with $T_d$, which is at $y_1=y_2 = Y^{\star}$ where \begin{align}
    Y^{\star} = -\frac{(p+q)2^{p+q}}{\sqrtsign{2}}u_D.
\end{align}
Let us also use $(X^{\clubsuit}, Y^{\clubsuit})$ for the point at which $T_h$ and $T_d$ intersect.

It is natural to consider the cases \begin{enumerate}[label=(\roman*)]
    \item $u_G < -u_D ~(Y^{\star} \text{ above } T_h)$
    \item $u_G > -u_D ~(Y^{\star} \text{ below }T_h)$
\end{enumerate}
and also \begin{enumerate}[label=(\alph*)]
    \item $u_G < 0 $
    \item $u_G > 0. $
\end{enumerate}
These cases are illustrated in Figure \ref{fig:phi_cases}. The first two quadratic terms in (\ref{eq:phi_outside}-\ref{eq:phi_inside}) determine the size of $\Phi$ when $y_2$ is `large enough' (which, in reality, will not be particularly large when compared with unity). So, for minimising $\Phi$ it is instructive to consider minimising $|y_2|$ and $|y_1 - y_2|$, hence the significance of $Y^{\star}.$ \begin{itemize}
    \item Referring to Figure \ref{fig:case_ia} we see that $|y_2|$ and $|y_1 - y_2|$ are jointly minimised in case (ia) at the top left corner of $B$ (denoted with a cross). \item In case (ib), shown in Figure \ref{fig:case_ib}, the minimising point is less apparent but lies on $T_d$; we indicate an illustrative poisition with a cross in the figure. 
    \item In case (iia), shown in Figure \ref{fig:case_iia}, a finite segment of $y_2 = y_1$ lies within $B$ and so clearly the joint minimising point is the intersection of $y_2 = y_1$ and $T_h$ denoted by a cross in the figure.
    \item Finally for case (iib), shown in Figure \ref{fig:case_iib} the joint minimising point is clearly at $y_2=y_1=0$.\end{itemize}
    
    Note that we have been considering only the first two quadratic terms in (\ref{eq:phi_outside}-\ref{eq:phi_inside}) and so the above indicated minimising points are not exact in all cases. $\Phi$ can be exactly minimised at the indicated point in case (ia) so long as $|u_G|$ is large enough that the first two quadratic terms in (\ref{eq:phi_outside}-\ref{eq:phi_inside}) are dominant over all the other terms. The same is true for case (iia). We expect cases (ib) and (iib) to be different, with the exact minimising point of $\Phi$ being modified from the points indicated in Figures \ref{fig:case_ib}, \ref{fig:case_iib} since $y_2$ is small at those points. Case (iib) is the only case where we expect the minimum of $\Phi$ on $B$ to be attained at a stationary point of $\Phi$, and we note that $\nabla\Phi=0$ exactly at $y_1=y_2=0$, so in case (iib) $\Phi$ is minimised on $B$ exactly at the origin. Let us summarise \begin{itemize}
        \item In case (iib) we know that $\Phi$ is minimized in $B$ at the origin and so we have the precise leading order term in the saddle point expansion.
        \item For large enough negative $u_G$ we know that $\Phi$ is minimized on $B$ at $(X^{\clubsuit}, Y^{\clubsuit})$ in case (ia) and at $y_1 = y_2 = Y^{\star}$ in case (iia). We do not however have a precise notion of what `large enough' is. 
    \end{itemize}

 We show contour plots of $\Phi$ for some fairly arbitrary parameter values in Figures \ref{fig:phi_sub}-\ref{fig:phi_super2} appearing to show the behaviour of cases (ia), (iia) and (ib). We have also seen (iib) but the plots are much less informative.\\
 

    \begin{figure*}
        \centering
        \begin{subfigure}[b]{0.475\textwidth}
            \centering
    \begin{tikzpicture}
    \draw[step=1cm,gray,very thin] (-1.9,-1.9) grid (5.9,5.9);
    \draw[dotted, thick] (-1.9,2)--(5.9,2);
    \draw[red, thick] (-1.9,0)--(5.9,0);
    \node at (6.2, 0){$T_h$};
    \draw[red, thick] (-1, -1.9)--(4, 5.9);
    \node at (4.2, 5.7){$T_d$};
    \draw[fill=red, nearly transparent]  (0.2,0) -- (5.9,0) -- (5.9, -1.9) -- (-1,-1.9) -- cycle;
    \node at (0.2, 0){$\times$};
    \node at (3, -1){$B$};
    \draw[thick, dash dot, black] (-1.9, -1.9)--(5.9,5.9);
    \node at (0.8, 0.3){$Y^{\star}$};
    \end{tikzpicture}
    \caption{Case (ia).}
            \label{fig:case_ia}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}  
            \centering 
    \begin{tikzpicture}
    \draw[step=1cm,gray,very thin] (-1.9,-1.9) grid (5.9,5.9);
    \draw[dotted, thick] (-1.9,2)--(5.9,2);
    \draw[red, thick] (-1.9,3)--(5.9,3);
    \node at (6.2, 3){$T_h$};
    \draw[red, thick] (1.8, -1.9)--(5.5, 5.9);
    \node at (5, 5.7){$T_d$};
    \draw[fill=red, nearly transparent]  (4.1,3) -- (5.9,3) -- (5.9, -1.9) -- (1.8,-1.9) -- cycle;
            \node at (3.8, 2.3){$\times$};
    \node at (3, -1){$B$};
    \draw[thick, dash dot, black] (-1.9, -1.9)--(5.9,5.9);
    \node at (0.8, 0.3){$Y^{\star}$};
    \end{tikzpicture}
    \caption{Case (ib).}
            \label{fig:case_ib}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
    \begin{tikzpicture}
    \draw[step=1cm,gray,very thin] (-1.9,-1.9) grid (5.9,5.9);
    \draw[dotted, thick] (-1.9,2)--(5.9,2);
    \draw[red, thick] (-1.9,1)--(5.9,1);
    \node at (6.2, 1){$T_h$};
    \draw[red, thick] (-1, -1.9)--(2.5, 5.9);
    \node at (2.7, 5.7){$T_d$};
    \draw[fill=red, nearly transparent]  (0.285,1) -- (5.9,1) -- (5.9, -1.9) -- (-1,-1.9) -- cycle;
    \node at (3, -1){$B$};
    \draw[thick, dash dot, black] (-1.9, -1.9)--(5.9,5.9);
        \node at (1, 1){$\times$};
    \node at (0.8, 0.3){$Y^{\star}$};
    \end{tikzpicture}
    \caption{Case (iia).}
            \label{fig:case_iia}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
    \begin{tikzpicture}
    \draw[step=1cm,gray,very thin] (-1.9,-1.9) grid (5.9,5.9);
    \draw[dotted, thick] (-1.9,2)--(5.9,2);
    \draw[red, thick] (-1.9,3)--(5.9,3);
    \node at (6.2, 3){$T_h$};
    \draw[red, thick] (-1, -1.9)--(4, 5.9);
    \node at (4.2, 5.7){$T_d$};
    \draw[fill=red, nearly transparent]  (2.14,3) -- (5.9,3) -- (5.9, -1.9) -- (-1,-1.9) -- cycle;
        \node at (2, 2){$\times$};
    \node at (3, -1){$B$};
    \draw[thick, dash dot, black] (-1.9, -1.9)--(5.9,5.9);
    \node at (0.8, 0.3){$Y^{\star}$};
    \end{tikzpicture}
    \caption{Case (iib).}
            \label{fig:case_iib}
        \end{subfigure}
        \caption{Cases for the minimisation of $\Phi$ shown in $(y_1, y_2)$ plane. Horizontal dotted line denotes $y_2 = 0$ and diagonal dot-dashed line denotes $y_2 = y_1$.}
        \label{fig:phi_cases}
    \end{figure*}



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{bivariate_exponent_contour_subcrit.pdf}
    \caption{Numerical example of the minimum of $\Phi$ being attained at $(X^{\clubsuit}, Y^{\clubsuit})$ (i.e. top left of $B$) as in case (ia). White denotes regions outside $B$.}
    \label{fig:phi_sub}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{bivariate_exponent_contour_supercrit.pdf}
  \caption{Numerical example of the minimum of $\Phi$ being attained on $T_d$ as in case (ib). White denotes regions outside $B$. }    \label{fig:phi_super}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{bivariate_exponent_contour_supercrit2.pdf}
  \caption{Numerical example of the minimum of $\Phi$ being attained on $T_h$ as in case (iia). White denotes regions outside $B$.}    \label{fig:phi_super2}
\end{figure}

 We propose that the correct notion of `large enough' negative $u_G$ comes from requiring $\partial_{y_2} \Phi < 0$ for all $(y_1, y_2)\in B$. First consider $|y_1| > r$. Simple differentation reveals that \begin{align}\label{eq:dphidy2_out}
     \frac{\partial \Phi}{\partial y_2} = \frac{2\left(s^{-2} + 2p^{-2}\right)y_2^2 + \left(\left(s^{-2} + 2p^{-2}\right)\eta^{-1}c(y_1) - 2p^{-2}y_1\right)y_2 - 2\left(p^{-2}\eta^{-1}y_1c(y_1) + \kappa'\right)}{2y_2 + \eta^{-1}c(y_1)}
 \end{align}
 where we have defined \begin{align}\label{eq:c_def}
  c(y) = -y + \text{sgn}(y)\sqrtsign{y^2 - r^2}.
\end{align}
We first consider the level sets of the denominator of (\ref{eq:dphidy2_out}, in particular \begin{align}
    2y_2 + \eta^{-1}c(y_1) = 0\label{eq:hyperbola}.
\end{align}
Simple manipulation of (\ref{eq:hyperbola}) gives \begin{align}
  \frac{1}{4}y_2^2 -  \left(y_2 - \frac{1}{2}y_1\right)^2   = \frac{r^2}{4\eta^2}
\end{align}
which defines an hyperbola with asymptotes $y_2 = 0$, $y_2 = y_1$ and vertices $y_1 = \pm \frac{r}{\eta}$ -- see Figure \ref{fig:hyperbola}. Note that $\eta > 1$ and so $0< \frac{r}{\eta} < r$. Clearly, taking $y_2 \rightarrow -\infty$ gives \begin{align}
    2y_2 + \eta^{-1}c(y_1) < 0
\end{align}
and so we can conclude that \begin{equation}
     2y_2 + \eta^{-1}c(y_1) < 0, ~~~ y_2 < 0, ~ y_1 > y_2.
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{hyperbola.pdf}
    \caption{The critical hyperbola for determining the sign of $\partial_{y_2}\Phi$.}
    \label{fig:hyperbola}
\end{figure}

We now must consider the numerator of (\ref{eq:dphidy2_out}). First consider the case $y_1\rightarrow - \infty$, where $c(y_1)\sim -\frac{r^2}{2y_1}$ and so the numerator gives a quadratic with roots satisfying \begin{align}
    2\left(2p^{-2} + s^{-2}\right)y_2^2 - 2p^{-2}y_1y_2 - \left(2\kappa' - \eta^{-1}p^{-2}r^2\right) = 0.\label{eq:dphi_sign_quadratic}
\end{align}
As $y_1\rightarrow - \infty$, the roots of (\ref{eq:dphi_sign_quadratic}) are \begin{align}
    y_2 \sim \frac{p^{-2}}{2p^{-2} + s^{-2}} y_1, ~~ y_2 \sim \mathcal{O}(y_1^{-1}).
\end{align}
Note that $\frac{p^{-2}}{2p^{-2} + s^{-2}} < \frac{1}{2}$ and so, for large negative $y_1$, we conclude that $\partial_{y_2}\Phi < 0$ if $y_1 > y_2$. Further, this conclusion is in fact valid up to the smallest root of \begin{align}
  2\left(s^{-2} + 2p^{-2}\right)y^2 + \left(\left(s^{-2} + 2p^{-2}\right)\eta^{-1}c(y) - 2p^{-2}y\right)y - 2\left(p^{-2}\eta^{-1}yc(y) + \kappa'\right) = 0.\label{eq:y_sqr_quad}
\end{align}

Numerical solution of (\ref{eq:y_sqr_quad}) for a wide variety of values of $p,q,\sigma_z, \kappa$ indicates that it possess no real solutions for $y< -r.$ We therefore conclude that $\partial_{y_2}\Phi < 0$ for $|y_1| >r , y_2 < 0, y_2 < y_1$. Now consider $|y_1| < r$. We have \begin{align}
    \frac{\partial \Phi}{\partial y_1} &= -\frac{2y_2}{p^2} + \left(2p^{-2} - \frac{1}{2\eta^{-1}}\left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)\right)y_1 + \frac{2\kappa'\eta^{-1}y_2}{r^2\eta^{-1} + 4y_2^2 - 4\eta^{-1}y_1y_2}\notag\\
    & \overset{(a)}{>}-\frac{2y_2}{p^2} + \left(2p^{-2} - \frac{1}{2\eta^{-1}}\left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)\right)y_1 + \frac{2\kappa'\eta^{-1}y_2}{(2y_2 + \eta^{-1}r)^2}\notag\\
    &  \overset{(b)}{>}  -\frac{2y_2}{p^2} -r\left|2p^{-2} - \frac{1}{2\eta^{-1}}\left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)\right| + \frac{2\kappa'\eta^{-1}y_2}{(2y_2 + \eta^{-1}r)^2}.
\end{align}
The inequality (a) follows from observing that the denominator of the last term on the first line is strictly positive for all $y_2$ and all $|y_1| < r$ and then minimising that denominator over $|y_1| < r$. Inequality (b) follows simply from minising the middle term over $|y_1| < r$. If follows that $\partial_{y_1}\Phi > 0$ for all $|y_1| < r$ and $y_2 < 0$ if \begin{align}\label{eq:dphi_dy1_pos_cond}
2\left(p^{-2} - \kappa'\eta^{_1}\left(2y_2 +\eta^{-1}r\right)^{-2}\right)y_2 < -r \left|2p^{-2} - \frac{1}{2\eta^{-1}\left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)}\right|.
\end{align}
If we take \begin{align}\label{eq:y2_p2_bound}
    \left(2y_2 + r\eta^{-1}\right)^{-2}\kappa'\eta^{-1} < \frac{1}{2}p^{-2} ~~ \iff ~~ y_2 < -\left(\frac{\sqrtsign{2\kappa'\eta^{-1}p^2} - \eta^{-1}r}{2}\right)
\end{align}
then \begin{align}
    -\frac{r}{2}\left|2p^{-2} - \frac{1}{2\eta^{-1}\left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)}\right|\left(p^{-2} - \kappa\eta^{-1}\left(2y_2 - r\eta^{-1}\right)^{_2}\right)^{-1} < -rp^2\left|2p^{-2} - \frac{1}{2\eta^{-1}\left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)}\right|
\end{align}
and so a sufficient condition for (\ref{eq:dphi_dy1_pos_cond}) is \begin{align}
    y_2 < -rp^2\left|2p^{-2} - \frac{1}{2\eta^{-1}\left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)}\right|.
\end{align}
Overall, a sufficient condition for (\ref{eq:dphi_dy1_pos_cond}) is \begin{align}
    y_2 < -\max\left\{\left(\frac{\sqrtsign{2\kappa'\eta^{-1}p^2} - \eta^{-1}r}{2}\right), rp^2\left|2p^{-2} - \frac{1}{2\eta^{-1}\left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)}\right|\right\}
\end{align}

We now repeat this analysis for $\partial_{y_2}\Phi$. We have \begin{align}
    \frac{\partial \Phi}{\partial y_2} &= \frac{2y_2}{p^2} + \frac{y_2}{s^2} - \frac{2y_1}{p^2}  + \frac{2\kappa'\eta^{-1}y_1 - 4\kappa'y_2}{r^2\eta^{-1} + 4y_2^2 - 4\eta^{-1}y_1y_2}\notag\\
    & < \frac{2y_2}{p^2} + \frac{y_2}{s^2}
    - \frac{4\kappa'y_2}{(2y_2 + \eta^{-1}r)^2} +\frac{2\kappa'\eta^{-1}r }{(2y_2 + \eta^{-1}r)^2} + \frac{2r}{p^2} .
\end{align}
We need to bound $y_2$ away from $-\frac{r}{2\eta}$, so say $y_2 < -\alpha\frac{r}{2\eta}$ for some $\alpha >1$. It then follows that \begin{align}
     \frac{\partial \Phi}{\partial y_2} & <  \frac{2y_2}{p^2} + \frac{y_2}{s^2}
    2\kappa'\eta r^{-1} (1-\alpha)^{-2}\alpha + 2\kappa'\eta r^{-1} (1-\alpha)^{-2} + \frac{2r}{p^2}
\end{align}
and so sufficient for $\partial_{y_2}\Phi < 0$ is \begin{align}
    y_2 < -\max\left\{\frac{r\alpha}{2\eta}, \frac{2\kappa'\eta r^{-1} (1-\alpha)^{-2} (\alpha + 1) + 2rp^{-2}}{2p^{-2} + s^{-2}}\right\}.
\end{align}
Optimising this upper bound over $\alpha > 1$ amounts to finding the unique $\alpha> 1$ satisfying \begin{align}
    \frac{r\alpha}{2\eta}= \frac{2\kappa'\eta r^{-1} (1-\alpha)^{-2} (\alpha + 1) + 2rp^{-2}}{2p^{-2} + s^{-2}}
\end{align}
so $\alpha$ is given as the largest root of \begin{align}
    \alpha^3 - \left[2 + 4\eta p^{-2}(s^{-2} + 2p^{-2})\right]\alpha^2 &+ \left[1 + 8\eta p^{-2} (2p^{-2} + s^{-2})^{-1} - 4\kappa' \eta^2 r^{-2}(2p^{-2} + s^{-2})^{-1}\right]\alpha \notag\\
    &- 4\eta r^{-1}(2p^{-2} + s^{-2})^{-1}\left(r p^{-2} + \kappa'\eta r^{-1}\right) = 0.
\end{align}


Let us now suppose that \begin{align}
    u_G < \frac{\sqrtsign{2}}{p+q} 2^{-p-q}\max\left\{\left(\frac{\sqrtsign{2\kappa'\eta^{-1}p^2} - \eta^{-1}r}{2}\right), rp^2\left|2p^{-2} - \frac{1}{2\eta^{-1}\left(b^{-2} + b_1^{-2}(\eta - 1)^2\right)}\right|, - \frac{r\alpha}{2\eta} \right\}
\end{align}
so that, from the preceding discussion, $\partial_{y_2}\Phi < 0$ in $B$ for all $y_1$ and $\partial_{y_1}\Phi > 0$ in $B$ for $|y_1| < r$. It is therefore clear that, the case (ia) applies. 

\begin{comment}
For $|y_1| < r$ simple differentiation establishes that $\partial_{y_2}\Phi < 0$ if and only if \begin{align}\label{eq:y2_cond_in}
    \frac{\left( y_2 s^{-2} + (y_2 - y_1)p^{-2}\right)\left(r^2\eta^{-2} + 4y_2^2 - 4\eta^{-1}y_1y_2\right) - 2\kappa'(2y_2 - \eta^{-1}y_1)}{r^2\eta^{-2} + 4y_2^2 - 4\eta^{-1}y_1y_2}<0.
\end{align}
The denominator of (\ref{eq:y2_cond_in}) can be easily seen to positive for all $|y_1|<r$ and all $y_2$.The numerator defines a cubic in $y_2$:\begin{align}
    &4\left[s^{-2} + p^{-2}\right]y_2^3  -4\left[p^{-2}y_1 + \eta^{-1}(p^{-2} + s^{-2})y_1\right]y_2^2 \notag\\
    &+ \left[r^2\eta^{-2}(s^{-2} + p^{-2}) +4\eta^{-1}p^{-2}y_1^2- 4\kappa'\right]y_2 + \left[2\kappa'\eta^{-1}y_1 - r^2\eta^{2}p^{-2}y_1\right] = 0\label{eq:y2_cubic}
\end{align}
For $|t| < r$ define $\psi(t)$ to be the smallest real root of (\ref{eq:y2_cubic}. Repeating the above procedure for $|y_1| > r$ results in a denominator   \begin{align}\label{eq:y2_c_constraint}
    \frac{1}{\eta}\left(-y_1 + \text{sgn}(y_1)\sqrtsign{y_1^2 - r^2}\right) + 2y_2 \equiv \frac{1}{\eta}c(y_1) + 2y_2
\end{align} and the numerator defines a quadratic \begin{align}
    2\left[s^{-2} + p^{-2}\right]y_2^2 + \left[\eta^{-1}c(y_1) - 2p^{-2}y_1\right]y_2 -\left[ p^{-2}\eta^{-1}y_1c(y_1) + 2\kappa'\right] = 0.\label{eq:y2_quadratic}
\end{align}
For $t\leq -r$ define $\psi(t)$ to be the least real root of (\ref{eq:y2_quadratic}) if it exists, or else $\psi(t) = -\frac{1}{2\eta}c(y_1).$ With $\psi$ so defined, we claim that $\psi$ intersects $T_d$ exactly once and we take $t_{\psi}$ to be the solution, i.e. $(t_{\psi}, \psi(t_{\psi}))\in T_d$. Therefore the sought notion of `large enough negative' $u_G$ is given by \begin{align}
    u_G < \frac{\sqrtsign{2}}{(p+q)2^{p+q}}t_{\psi}\equiv E_{G}.
\end{align}
Note that $t_{\psi}$ is a function of $u_D$.
The regions (ia) and (iia) are further divided into (iaI), (iaII), (iiaI) and (iiaII) according to $|y_1| > r$ or $|y_1| < r$. We now consider the $(u_D, u_G)$ plane. We have the bounding lines $u_G = -u_D$ and $u_G =0$ defining the four regions in which cases (ia), (ib), (iia) and (iib) apply. Region (iia) is divided along \begin{align}
    u_G = -\frac{\sqrtsign{2}r}{(p+q)2^{p+q}}
\end{align}
with (iiaII) above and (iiaI) below. Region (ia) is divided along \begin{align}
    u_G = \left(pu_D \pm \sqrtsign{2}r\right)\left( (p+q)2^{p+q} - p\right)^{-1}
\end{align}
with (iaII) lying between the two lines and (iaI) outside. We know have the ingredients to plot some details of the $u_D, u_G$ plane and to plot the minimum value of $\Phi$ in $B$ (i.e. the value of interest) as a function of $u_D, u_G$ in some subset of the plane. Figure \ref{fig:u_plane_regions} shows an example of the regions of the $u_D, u_G$ plane and Figure \ref{fig:u_plane_phi} shows the corresponding partial plot of the minimum of $\Phi$ on $B$.
\end{comment} 


\begin{figure}
    \centering
    \includegraphics{u_plane_regions}
    \caption{Regions of the $u_D, u_G$ defined by the location of the minimum point of $\Phi$ in $B$. The white region denotes cases not covered by (ia), (ib), (iia), (iib), namely where $u_G\in (t_{\psi}, 0)$.}
    \label{fig:u_plane_regions}
\end{figure}

\begin{figure}
    \centering
    \includegraphics{phi_in_u_plane}
    \caption{Minimum of $\Phi$ in $B$ plotted in the $u_D, u_G$ plane. The white region denotes cases where the minimum is not analytically tranctable.}
    \label{fig:u_plane_phi}
\end{figure}
 \subsection{Prescribed Hessian index}
 The natural quantity of interest is \begin{align}
    C_{N, k_D, k_G} =\Bigg|\Bigg\{ \vwD\in S^{N_D  }, \vwG\in S^{N_G } ~:~ &\nabla_D \LD = 0, \nabla_G \LG = 0, \LD\in B_D, \LG\in B_G\notag\\
    &i(\nabla_D^2 L^{(D)}) = k_D, ~i(\nabla_G^2 L^{(G)}) = k_G \Bigg\}\Bigg|\label{eq:C_Nkk_def}
\end{align}
and, in particular, $\log\mathbb{E} C_{N, k_D, k_G}$.
The extra Hessian signature conditions in (\ref{eq:C_Nkk_def}) enforce that both generator and discriminator are at low-index saddle points. To compute this quantity, we meet the same difficulty encountered in \cite{baskerville2020loss}, namely that, when using the supersymmetric representation as in the preceding subsection, in going from (\ref{eq:no_hessian_k_delta}) to (\ref{eq:no_hessian_k_expect_delta}) we have to compute the Fourier transform of a GOE distribution with an index constraint. The issue is further confounded here because we do not perform the supersymmetric Kac-Rice calculations directly with the natural Hessian matrix (\ref{eq:H_first}), but rather in the rewritten form (\ref{eq:symmetric-block-matrix}). We find however that we can indeed proceed much as in \cite{baskerville2020loss}. We first consider the problem of computing \begin{align}
    \mathbb{E}|\det H|\mathbbm{1}\left\{ i\left(\sqrtsign{\kappa}\sqrtsign{b^2 + b_1^2}M_D + \frac{x'+x_1'}{\sqrtsign{2N}}\right) = k_D, ~ i\left(\sqrtsign{\kappa'}bM_G - \frac{x'}{\sqrtsign{2N}}\right) = k_G\right\}
\end{align}
where $H$ is given as in (\ref{eq:H_first}) by \begin{align}
    H =  \left(\begin{array}{cc}
      \sqrtsign{2\kappa N}\sqrtsign{b^2 + b_1^2}M^{(D)} & -bG \\
       b G^T & \sqrtsign{2\kappa'N}bM^{(G)}
    \end{array}\right)
   -x' \left(\begin{array}{cc}
        -I_{N_D} & 0  \\
         0 & I_{N_G} 
    \end{array}\right)  + x_1'\left(\begin{array}{cc}
        I_{N_D} & 0  \\
         0 & 0
    \end{array}\right)
\end{align}
where $M^{(D)}\sim GOE^{\kappa N}$, $M^{(G)}\sim GOE^{\kappa' N}$, $G$ is $\kappa N \times \kappa' N$ Ginibre and all are independent. Let us now move to the supersymmetric representation as in (\ref{eq:no_hessian_k_delta}). The crux of the matter is that we must compute \begin{align}
   & \mathbb{E}_{M^{(D)}}e^{-i\sqrtsign{\kappa} \sqrtsign{b^2 + b_1^2}\Tr M^{(D)} A[1]}\mathbbm{1}\left\{i\left(M_D + \frac{x' + x_1'}{\sqrtsign{\kappa}\sqrtsign{b^2 + b_1^2}}\right) = k_D\right\},\\
      & \mathbb{E}_{M^{(G)}}e^{-i\sqrtsign{\kappa'} b \Tr M^{(G)} A[2]}\mathbbm{1}\left\{i\left(M_G - \frac{x'}{\sqrtsign{\kappa'}b}\right) = k_G\right\},
\end{align}
but \cite{baskerville2020loss} has performed exactly these calculations (see around (5.146) therein) and so there exist constants $K^{(D)}_U,K^{(D)}_L, K^{(G)}_U,K^{(G)}_L$ such that \begin{align}
  &K^{(D)}_L e^{-Nk_D\kappa(1 + o(1)) I_1(\hat{x}_D; \sqrtsign{2})} e^{-\frac{1}{2N}(b^2 + b_1^2)\Tr A[1]^2}  \notag\\
  \leq  &\Re\mathbb{E}_{M^{(D)}}e^{-i\sqrtsign{\kappa} \sqrtsign{b^2 + b_1^2}\Tr M^{(D)} A[1]}\mathbbm{1}\left\{i\left(M_D + \frac{x' + x_1'}{\sqrtsign{\kappa}\sqrtsign{b^2 + b_1^2}}\right) = k_D\right\} \notag\\
  \leq &K^{(D)}_U e^{-Nk_D\kappa(1 + o(1)) I_1(\hat{x}_D; \sqrtsign{2})} e^{-\frac{1}{2N}(b^2 + b_1^2)\Tr A[1]^2}
\end{align}
and 
\begin{align}
  &K^{(G)}_L e^{-Nk_G\kappa'(1 + o(1)) I_1(\hat{x}_G; \sqrtsign{2})} e^{-\frac{1}{2N}b^2 \Tr A[2]^2}  \notag\\
  \leq  &\Re\mathbb{E}_{M^{(G)}}e^{-i\sqrtsign{\kappa'} b\Tr M^{(G)} A[2]}\mathbbm{1}\left\{i\left(M_G - \frac{x'}{\sqrtsign{\kappa'}b}\right) = k_G\right\} \notag\\
  \leq &K^{(G)}_U e^{-Nk_G\kappa'(1 + o(1)) I_1(\hat{x}_G; \sqrtsign{2})} e^{-\frac{1}{2N}b^2 \Tr A[2]^2}
\end{align}
where \begin{align}
    \hat{x}_D = -\frac{x' + x_1'}{\sqrtsign{\kappa}\sqrtsign{b^2 + b_1^2}}, ~~ \hat{x}_G = \frac{x'}{\sqrtsign{\kappa'}b}.
\end{align}
Here $I_1$ is the rate function of the largest eigenvalue of the GOE as obtained in \cite{arous2001aging} and used in \cite{auffinger2010random, baskerville2020loss}: \begin{align}
    I_1(u; E) = \begin{cases} \frac{2}{E^2}\int_u^{-E} \sqrtsign{z^2 - E^2}dz ~ &\text{ for } u < -E,\\
        \frac{2}{E^2}\int_{E}^u \sqrtsign{z^2 - E^2}dz ~ &\text{ for } u > E,\\
    \infty &\text{ for } |u| < E.
    \end{cases}
\end{align}
Note that for $u< -E$ \begin{align}
    I_1(u; E) = -\frac{u}{E}\sqrtsign{u^2 - E^2} - \log\left(-u + \sqrtsign{u^2 - E^2}\right) + \log{E}
\end{align}
and for $u>E$ we simply have $I_1(u; E) = I_1(-u; E)$.\\


We have successfully dealt with the Hessian index indicators inside the expectation, however we need some way of returning to the form of $H$ in (\ref{eq:H_rewritten}) so that the supersymmetric calculations of the previous section can be followed through. We can achieve this with inverse Fourier transforms:
\begin{align}
    e^{-\frac{1}{2N}(b^2 + b_1^2)\Tr A[1]^2} &= \mathbb{E}_{M_D}e^{-i\sqrtsign{\kappa}\sqrtsign{b^2 + b_1^2}\Tr M_DA[1]}\\
     e^{-\frac{1}{2N}b^2\Tr A[2]^2} &= \mathbb{E}_{M_G}e^{-i\sqrtsign{\kappa'}b\Tr M_GA[2]}   
\end{align}
from which we obtain \begin{align}
&K_Le^{-Nk_D\kappa(1 + o(1)) I_1(\hat{x}_D; \sqrtsign{2})} e^{-\frac{1}{2N}(b^2 + b_1^2)\Tr A[1]^2}e^{-Nk_G\kappa'(1 + o(1)) I_1(\hat{x}_G; \sqrtsign{2})}\mathbb{E}|\det H|\notag\\
\leq 
  & \mathbb{E}|\det H|\mathbbm{1}\left\{ i\left(\sqrtsign{\kappa}\sqrtsign{b^2 + b_1^2}M_D + \frac{x'+x_1'}{\sqrtsign{2N}}\right) = k_D, ~ i\left(\sqrtsign{\kappa'}bM_G - \frac{x'}{\sqrtsign{2N}}\right) = k_G\right\} \\
  \leq & K_Ue^{-Nk_D\kappa(1 + o(1)) I_1(\hat{x}_D; \sqrtsign{2})} e^{-\frac{1}{2N}(b^2 + b_1^2)\Tr A[1]^2}e^{-Nk_G\kappa'(1 + o(1)) I_1(\hat{x}_G; \sqrtsign{2})} \mathbb{E}|\det H|
  \end{align}
and so the saddle point exponent function $\mathcal{L}(y_1, y_2)$ from the previous section is modified to include two extra terms \begin{align}\label{eq:l_kd_kg}
    \mathcal{L}_{k_D, k_G} = \mathcal{L}(y_1, y_2) + \left[k_D\kappa I_1(-y_1; \sqrtsign{2\kappa(b^2 + b_1^2)}) + k_G\kappa' I_1(y_2; \sqrtsign{2\kappa'}b)\right].
\end{align}

Recalling the analysis of the preceding section, we have now to consider $\mathcal{L}_{k_D, k_G}$ on the domain $B$ to determine the leading order behaviour of  $\log\mathbb{E} C_{N, k_D, k_G}$. The extra GOE rate function terms in (\ref{eq:l_kd_kg}) further restrict the relevant $(y_1, y_2)$ domain to $B\cap \{(y_1, y_2) ~:~ |y_1| > \sqrtsign{2\kappa(b^2 + b_1^2)}, ~ |y_2| > \sqrtsign{2\kappa'} b\}$.
\end{comment}




% \section{Free probability approach}
% Recall the expression in (\ref{eq:H_rewritten}). It can be written as the absolute value of the characteristic polynomial of the following matrix \begin{align}
%     \mathcal{M} = bM + b_1\left(\begin{array}{cc} M_1 & 0 \\ 0 & 0 \end{array}\right) - \xi \left(\begin{array}{cc} 0 & 0 \\ 0 & I \end{array}\right)
% \end{align}
% where $\xi$ will be taken to be some fixed real number for now, and again $M_1\sim GOE^{\kappa N}, M\sim GOE^N$. Let $\mu_1$ denote the limiting spectral measure of \begin{align}
%     b_1\left(\begin{array}{cc} M_1 & 0 \\ 0 & 0 \end{array}\right) + \xi \left(\begin{array}{cc} 0 & 0 \\ 0 & I \end{array}\right).
% \end{align}
% As in \cite{biane1997free} we define \begin{align}
%     \lambda_t(dx) = \frac{1}{2\pi t} \sqrtsign{4t - x^2} dx
% \end{align}
% and then we have \begin{align}
%     \mu_1 = \kappa\lambda_{\frac{b_1^2}{2}} + (1-\kappa) \delta_{\xi}
% \end{align}
% where $\delta_{\xi}$ is a Dirac delta centred at $\xi$. The limiting spectral measure of $\mathcal{M}$ is therefore given by \begin{align}
%     \mu = \lambda_{\frac{b^2}{2}} \boxplus \mu_1 =  \lambda_{\frac{b^2}{2}} \boxplus \left(\kappa\lambda_{\frac{b_1^2}{2}} + (1-\kappa) \delta_{\xi}\right).
% \end{align}
% Following \cite{biane1997free} we set $t = \frac{b^2}{2}$ and we need to compute the set \begin{align}
%     U_t = \left\{u\in\mathbb{R} ~|~ \int\frac{d\mu_1(x)}{(u-x)^2} > \frac{1}{t}\right\} 
% \end{align} and the function \begin{align}
%     v_t(u) = \inf\left\{v\geq 0 ~|~ \int_{\mathbb{R}}\frac{d\mu_1(x)}{(u-x)^2 + v^2} \leq \frac{1}{t}\right\}
% \end{align}
% and thence the function \begin{align}
%     \psi_t(u) =u + t\int_{\mathbb{R}} \frac{(u-x)d\mu_1(x)}{(u-x)^2 + v_t(u)^2}
% \end{align}
% and then we have the following expression for the desired measure $\mu$ \begin{align}\label{eq:density_v_psi}
%     p(\psi_t(u)) = \frac{v_t(u)}{\pi t}
% \end{align}
% where $p$ is the density of $\mu$ with respect to the Lebesgue measure.



% \begin{lemma}\label{lemma:sc_conv_sc}
% For any $t, t' >0$
% \begin{align}
%     U_t^{t'} &\equiv \left\{u\in\mathbb{R} ~|~ \int\frac{d\lambda_{t'}(dx)}{(u-x)^2} > \frac{1}{t}\right\} = \left( -\sqrtsign{t+t'}, \sqrtsign{t+t'}\right),\\
%     v_t^{t'}(u)&\equiv \inf\left\{v\geq 0 ~|~ \int_{\mathbb{R}}\frac{d\lambda_{t'}(x)}{(u-x)^2 + v^2} \leq \frac{1}{t}\right\} = \sqrtsign{
%     (t+t') - u^2},\\
%     \psi_t^{t'}(u) &\equiv u + t\int_{\mathbb{R}} \frac{(u-x)d\lambda_{t'}(x)}{(u-x)^2 + v_t^{t'}(u)^2} = 2u
% \end{align}
% \end{lemma}
% \begin{proof}
% Let 
% Firstly note that  $\lambda_t \boxplus \delta = \lambda_t$ and let $  U_t^{(0)}, v_t^{(0)}, \psi_t^{(0)}$ denote the objects corresponding the free convolution of $\lambda_t$ and $\delta$ So \begin{align}
%  \frac{1}{2\pi t} \sqrtsign{4t - \psi_t^{(0)}(u)^2} = \frac{v_t^{(0)}(u)}{\pi t} ~~~ \implies ~~~ \frac{1}{2}\sqrtsign{4t - \psi_t^{(0)}(u)^2} = v_t^{(0)}(u).
% \end{align}
% But also \begin{align}
%     v_t^{(0)}(u) = \inf\left\{ v \geq 0 ~|~ (u^2 + v^2)
%     \leq t\right\} = \sqrtsign{t - u^2}
% \end{align}
% and so \begin{align}
%     \psi_t^{(0)}(u)^2 = 4\left(t - (t-u^2)\right) = 4u^2 ~~~ \implies \psi_t^{(0)}(u) = 2u.
% \end{align} But now notice that \begin{align}
%     \lambda_t \boxplus \lambda_{t'} = \lambda_{t+t'} = \lambda_{t+t'} \boxplus \delta
% \end{align}
% where the first equality can be established, e.g., concretely by considering the limiting spectral measure of the sum of two independent GOE matrices and recalling the additivity of the variances of independent Gaussians. The result follows immediately.
% \end{proof}

%  We have \begin{align}
%     \int\frac{d\mu_1(x)}{(u-x)^2 + v^2} = (1-\kappa)\left((\xi - u)^{2} + v^2\right)^{-1}+ \kappa \int\frac{d\lambda_{\frac{b_1^2}{2}}(x)}{(u-x)^2 + v^2}
% \end{align} 



% and so it would be useful to obtain a closed form expression (in terms of $v$) for \begin{align}
%   F(v, u) = \int\frac{d\lambda_{\frac{b_1^2}{2}}(x)}{(u-x)^2 + v^2}.
% \end{align}
% We have \begin{align}
%     \int\frac{d\lambda_{\frac{b_1^2}{2}}(x)}{(u-x)^2 + v^2} &= -\frac{1}{2iv} \int_{\mathbb{R}} d\lambda_{t'}\left(\frac{1}{iv + u -x} + \frac{1}{iv - u + x}\right)\notag\\
%     &= -\frac{1}{2iv}\left(G_{t'}(u + iv) + G_{t'}(-u + iv)\right)
% \end{align}
% noting that $v\geq 0$ and so $iv \pm u$ lies in the upper half plane, where $G_{t'}$ is defined, then \begin{align}
%     \int\frac{d\lambda_{\frac{b_1^2}{2}}(x)}{(u-x)^2 + v^2}
%     &= -\frac{1}{4ivt'}\left( 2iv - \sqrtsign{(u+iv)^2 - 4t'} - \sqrtsign{(u-iv)^2 - 4t'}\right)
% \end{align}
% where, as in \cite{biane1997free}, the square root is defined on $\mathbb{C} / \mathbb{R}_{+}$ with $\sqrtsign{-1} = i$. It follows that \begin{align}
%     \sqrtsign{(u+iv)^2 - 4t'} + \sqrtsign{(u-iv)^2 - 4t'} = \sqrtsign{R}\left(e^{i\theta/2} + e^{i(\pi - \theta/2)}\right)
% \end{align}
% where $R,\theta$ are the modulus and argument of $(u+iv)^2 - 4t'$, so \begin{align}
%     R^2 &= \left(u^2 - v^2 - 4t'\right)^2  + 4u^2v^2\\
%     \theta &= \sin^{-1}\frac{2uv}{R}
% \end{align}
% and we taken $\sin^{-1}$ in $[0,2\pi)$. Then \begin{align}
%       \int\frac{d\lambda_{\frac{b_1^2}{2}}(x)}{(u-x)^2 + v^2}
%     &= \frac{1}{2t'}\left( -1 + \sqrtsign{R}v^{-1}\sin\frac{\theta}{2}\right)\end{align}
% and so finally 
%  \begin{align}
%     \int\frac{d\mu_1(x)}{(u-x)^2 + v^2} = (1-\kappa)\left((\xi - u)^{2} + v^2\right)^{-1}+ \frac{\kappa}{2t'}\left( -1 + \sqrtsign{R}v^{-1}\sin\frac{\theta}{2}\right).\label{eq:V_argmin_function}
% \end{align} 
% A similar calculation gives \begin{align}
%     \int \frac{u-x}{(u-x)^2 + v_t(u)^2}d\lambda_{t'}(x) &= \frac{1}{2t'} \left(u + \sqrtsign{R(u)}\cos\frac{\theta(u)}{2}\right)
% \end{align}
% where we abusively write \begin{align}
%     R(u)^2 &= \left(u^2 - v_t(u)^2 - 4t'\right)^2  + 4u^2v_t(u)^2\\
%     \theta(u) &= \sin^{-1}\frac{2uv_t(u)}{R(u)}
% \end{align}
% and so \begin{align}
%     \psi_t(u) = u + \frac{t}{2t'} \left(u + \sqrtsign{R(u)}\cos\frac{\theta(u)}{2}\right) + \frac{t(1-\kappa)(u-\xi)}{(u-\xi)^2 + v_t(u)^2}.
% \end{align}





% \subsubsection{Old attempt - full supersymmetric treatment}
% In this section we will seek to combine the previous section with \cite{baskerville2020loss} to obtain leading order asymptotics for $C_N$. We begin with a supersymmetric expression for $|\det H|$ \cite{baskerville2020loss, fyodorov2004complexity}: \begin{align}
%     \mathbb{E} |\det H| = \lim_{\epsilon\rightarrow 0 } \Delta_{\epsilon} \equiv =\lim_{\epsilon\rightarrow 0} \frac{\det(H' - x - i\epsilon) \det(H' - x + i\epsilon)}{\sqrtsign{\det(H' - x - i \epsilon)}\sqrtsign{\det(H' - x + i\epsilon)}}
% \end{align}
% and \begin{align}
%     \de = \int d\Psi \exp\left\{ -\phi_1^{T}(x-H' + i \epsilon) \phi_1 -\phi_2^{T}(x-H' - i \epsilon) \phi_2 - i \chi_1^{\dagger}(x - H' + i\epsilon)\chi_1- i \chi_2^{\dagger}(x - H' - i\epsilon)\chi_2\right\}\end{align}
%  where the measure is \begin{align}
%      d\Psi =\prod_{j=1}^2  \frac{1}{\pi^{N/2} e^{-\frac{3\pi N i}{4}}}\prod_{t=1}^2 d\phi_j[t]d\chi_j[t] d\chi_j^*[t] =  \pi^{-N} e^{\frac{3\pi N i}{2}}\prod_{j=1}^2 \prod_{t=1}^2 d\phi_j[t]d\chi_j[t] d\chi_j^*[t],
%  \end{align}
% with $d\phi$ being the usual Lebesgue measure on $\mathbb{R}^{N}$ and $d\chi$ being Berezin integration measure over Grasmann variables.
% As before, taking expectations gives \begin{align}
%     \mathbb{E}\de &= \int d\Psi \exp\left\{-\frac{b^2}{2N} \trg Q^2 - \frac{b_1^2}{2\kappa N} \trg Q[1]^2 - ix_1\left(\psi[1]^{\dagger}\psi_1[1] + 
% \psi_2[1]^{\dagger}\psi_2[1]\right) - i
% \psi_1^{\dagger}(x + i\epsilon)\psi_1 - i \psi_2^{\dagger}(x - i\epsilon)\psi_2^{\dagger}\right\}
% \end{align}
%  where\begin{align}
%     \psi_j = \phi_j \otimes \left(\begin{array}{c} 1 \\ 0 \end{array}\right) + \chi_j \otimes \left(\begin{array}{c} 0 \\ 1 \end{array}\right)
% \end{align}
%  etc and \begin{align}
%      Q = \left(\begin{array}{cccccc}
% \phi_1^{\dagger}\phi_1 & \phi_1^{\dagger}\phi_2 & \phi_1^{\dagger}\chi_1 & 
% \phi_1^{\dagger}\chi_1^{*} & 
% \phi_1^{\dagger}\chi_2 & 
% \phi_1^{\dagger}\chi_2^{*} \\
% \phi_2^{\dagger}\phi_2 & \phi_2^{\dagger}\phi_2 & \phi_2^{\dagger}\chi_1 & 
% \phi_2^{\dagger}\chi_1^{*} & 
% \phi_2^{\dagger}\chi_2 & 
% \phi_2^{\dagger}\chi_2^{*} \\
% \chi_1^{\dagger}\phi_1 & \chi_1^{\dagger}\phi_2 & \chi_1^{\dagger}\chi_1 & 
% \chi_1^{\dagger}\chi_1^{*} & 
% \chi_1^{\dagger}\chi_2 & 
% \chi_1^{\dagger}\chi_2^{*} \\
% \chi_1^{T}\phi_1 & \chi_1^{\dagger}\phi_2 & \chi_1^{T}\chi_1 & 
% \chi_1^{T}\chi_1^{*} & 
% \chi_1^{T}\chi_2 & 
% \chi_1^{T}\chi_2^{*} \\
% \chi_2^{\dagger}\phi_1 & \chi_2^{\dagger}\phi_2 & \chi_2^{\dagger}\chi_1 & 
% \chi_2^{\dagger}\chi_1^{*} & 
% \chi_2^{\dagger}\chi_2 & 
% \chi_2^{\dagger}\chi_2^{*} \\
% \chi_2^{T}\phi_1 & \chi_1^{\dagger}\phi_2 & \chi_2^{T}\chi_1 & 
% \chi_2^{T}\chi_1^{*} & 
% \chi_2^{T}\chi_2 & 
% \chi_2^{T}\chi_2^{*} 
% \end{array}\right).
%  \end{align}
%  Performing two Hubbard-Stratonovich transformations \begin{align}
%      \expect\de &= \int d\Psi d\sigma d\sigma[1] \exp\left\{- \frac{N}{b^2} \trg \sigma^2 - \frac{\kappa N}{b_1^2} \trg \sigma[1]^2 - i\psi[1]^{\dagger}(\sigma[1] + x_1)\psi[1] - i \psi^{\dagger} (\sigma + x + i\epsilon S)\psi\right\}
%  \end{align}
%  where \begin{align}
%      \psi = \left(\begin{array}{r}
%      \phi_1 \\ \phi_2 \\ \chi_1 \\ \chi_1^* \\ \chi_2 \\ \chi_2^*
%      \end{array}\right), ~~~      \psi[1] = \left(\begin{array}{c}
%      \phi_1[1] \\ \phi_2[1] \\ \chi_1[1] \\ \chi_1[1]^* \\ \chi_2[1] \\ \chi_2[1]^*
%      \end{array}\right)
%  \end{align}
% and \begin{align}
%      S = \text{diag}\left(1, -1, 1, 0 ,-1, 0\right).
%  \end{align} Note that there is a  freedom in the definition of $S$: the first two components are fixed, but the last four can be any real $(s_1, s_2, s_3, s_4)$ such that $s_1 + s_2 = 1$ and $s_3 + s_4=-1$; we find the given choice convenient in what follows. Performing the straightforward Gaussian integrals now gives \begin{align}
%      \expect\de &= K_N' \int d\sigma d\sigma[1] \exp\left\{ - \frac{N}{b^2}\trg \sigma^2 - \frac{\kappa N}{b_1^2}\trg\sigma[1]^2 -\kappa N \trg \log \left(\sigma + \sigma[1] + x + x_1 + i\epsilon S\right) - \kappa' N \trg \log \left( \sigma +x + i\epsilon S\right)\right\}\label{eq:complexity_sigma_rep}
%  \end{align}
%  where \begin{align}
%      K_N' = \pi^{-N} e^{\frac{3\pi N i}{2}} (2\pi)^{6N} e^{-iN\pi} = 2^{6N} \pi^{5N} e^{\frac{iN\pi}{2}}.
%  \end{align}
 
%   At this point, we would like to diagonalise $\sigma$, absorb the diagonalising $U(2/4)$ matrix into $\sigma[1]$ and obtain diagonal saddle point equations for $\sigma, \sigma[1]$ as in the previous section, however the presence of the matrix $i\epsilon S$ precludes this approach precisely. We note however that in the $\epsilon\rightarrow 0$ limit, this term's only effect is to interact with the branch structure in the $(x,x_1)$ plane (c.f. \cite{baskerville2020loss}).  Diagonalising $\sigma, \sigma[1]$ would give integration variables of the form \begin{align}
%      \sigma &=\text{diag}\left(\sigma_1, \sigma_2, i\sigma_3, i\sigma_4, i\sigma_5, i\sigma_6\right),\\
%           \sigma[1] &
%           =\text{diag}\left(\sigma_1[1], \sigma_2[1], i\sigma_3[1], i\sigma_4[1], i\sigma_5[1], i\sigma_6[1]\right).
%  \end{align}
 
 
% We make the following key observations (valid in the limit $\epsilon\rightarrow 0$): \begin{enumerate}
%     \item Up-to the $\mathcal{O}(\epsilon)$ terms, $\sigma_3, \sigma_4, \sigma_5, \sigma_6,\sigma_3[1], \sigma_4[1], \sigma_5[1], \sigma_6[1]$ obey the same equations as $\sigma_{FF}, \sigma_{FF}[1]$ previously (with $x=z$).
%     \item $\sigma_1, \sigma_1[1]$ obey the same equations as $i\sigma_3, i\sigma_3[1]$. Similarly $\sigma_2, \sigma_2[1]$ obey the same equations as $i\sigma_5, i\sigma_5[1]$.
%     \item $\sigma_4, \sigma_4[1]$ obey the same equations as $\sigma_6, \sigma_6[1]$.
% \end{enumerate}


%  Proceeding analytically from this stage seems intractable. To do so, we would first have to introduce an explicit parametrisation of $U(2/4)$ and, more problematically, we would have to solve the saddle point equations and determine their branch structure in the $x, x_1$ plane.
 
%  At any $(x,x_1)$, we can compute numerically the 4 roots of the equations (\ref{eq:ferm_saddle1}-\ref{eq:ferm_saddle2}). Due to the above observations, we need only determine $\sigma_3, \sigma_4, \sigma_5$, since \begin{align}
%      \sigma_1 &= i\sigma_3\\ \sigma_2 &= i\sigma_5\\ \sigma_4 &= \sigma_6\\
%          \sigma_i[1] &= \frac{b_1^2}{2\kappa}\left(\frac{2}{b^2}\sigma_{i} - \kappa'(\sigma_{i} - ix)^{-1}\right), ~~ i=3,4,5,6.
%  \end{align} 
 
%  Writing \begin{align}
%      \expect\Delta_{\epsilon} = K_N'\int d\sigma d\sigma[1] e^{-N\Phi(x, x_1)}
%  \end{align}
%  we then have \begin{align}
%      \Phi|_{\text{saddle}} = \frac{2}{b^2} \sigma_4^2 + \frac{2\kappa}{b_1^2}\sigma_4[1]^2 - 2\kappa\sum_{i=3}^5 \log\left(\sigma_i + \sigma_i[1] -ix -ix_1\right)
%      - 2\kappa'\sum_{i=3}^5 \log\left(\sigma_i  -ix\right)
%  \end{align}
%  and so the overall complexity has leading order term \begin{align}
%   \log \mathbb{E}C_N \sim \log{K_N''} -N \left(-\frac{1}{2s^2}x_*^2 + \frac{1}{2s_1^2} (x_1)_*^2 + \Phi|_{\text{saddle}}(x_*, (x_1)_*)\right)
%  \end{align}
%  where \begin{align}
%      K_N'' = K_NK_N' \sqrtsign{\frac{N-2}{2\pi s_1^2}} \sqrtsign{\frac{N-2}{2\pi s^2}}
%  \end{align}
%  and $(x_*, (x_1)_*)$ is the saddle point location in $(x, x_1)$ space. The constant term has asymptotic form \begin{align}
%      \frac{1}{N}\log K_N'' \sim \frac{13}{2}\log{2} + 5\log{\pi} - \frac{\kappa}{2}\log\left(p + \sigma_z^22^{p+q}(p+q)\right) - \frac{\kappa'}{2} \log\left(\sigma_z^2(p+q) 2^{p+q}\right) - \frac{\kappa}{2}\log\kappa - \frac{\kappa'}{2}\log\kappa' + \frac{i\pi}{2}.
%  \end{align}






% \begin{theorem}
% Let $(H_N)_{N=1}^{\infty}$ be a sequence of random matrices, where for each $N$ \begin{align}
%     H_N \overset{d}{=}  bM + b_1\left(\begin{array}{cc}
%      M_1 & 0 \\ 0 & 0\end{array}\right) - x_1\left(\begin{array}{cc}
%      I & 0 \\ 0 & 0\end{array}\right)
% \end{align}
% and $M\sim GOE^N$, $M_1\sim GOE^{\kappa N}$. Then  \begin{align}
% \int_B dx dx_1 ~ e^{-N\left(\frac{x^2}{2s^2} + \frac{x_1^2}{2s_1^2}\right)}\mathbb{E} |\det(H_N-xI)| = (1 + o(1))\int_B dx dx_1 ~ \exp\left\{-N\left(\frac{x^2}{2s^2} + \frac{x_1^2}{2s_1^2} - \int \log|z - x| d\mu_{eq}(z)\right)\right\}
% \end{align}
%  as $N\rightarrow\infty$.
% \end{theorem}
% \begin{proof}
% Let $\mu_N$ be the empirical spectral measure of the $H_N$ and say $\mu_N\rightarrow \mu$ weakly almost surely. We begin by establishing an upper bound. For any $\alpha,\beta>0$ \begin{align}
%     \expect |\det (H-xI)| &= \expect\left[\exp\left\{N\int \log|z-x| d\mu_N(z)
%     \right\}\right] \notag\\
%     & \leq \underbrace{\left(\expect\left[\exp\left\{2N\int \max\left(-\alpha, \min\left(\log|x-z|, \beta\right)\right)\right\}\right]\right)^{1/2}}_{A_N} \underbrace{\left(\expect\left[\exp\left\{2N\int \log|x-z|\indic\{|x-z|\geq e^{\beta}\}\right\}\right]\right)^{1/2}}_{B_N}.
% \end{align}
% Considering $B_N$, we have \begin{align}
%     \log|x-z| \indic\{|x-z| \geq e^{\beta}\} \leq |x-z|\indic\{|x-z| \geq e^{\beta}\} \leq e^{-\beta}(x-z)^2
% \end{align}
% and so \begin{align}
%   \expect\left[\exp\left\{2N\int \log|x-z|\indic\{|x-z|\geq e^{\beta}\}\right\}\right] &\leq  \expect \left[\exp\left\{2N e^{-\beta} \frac{\Tr (H - xI)^2}{N}\right\}\right] \notag\\
%   &= \expect \left[\exp\left\{2e^{-\beta} \Tr (H - xI)^2\right\}\right]\notag\\
%   &\approx e^{N\mathcal{O}(e^{-\beta})}
% \end{align}
% which becomes unity in the limit $\beta\rightarrow\infty$. It is sufficient now to show \begin{align}
%     \expect \left[\exp\left\{ 2N \int f(z) d\mu_N(z)\right\}\right] = \exp\left\{2N\left(\int f(z) d\mu(z) + o(1)\right)\right\}
% \end{align}
% where $f(z) = 2\max\left(\min(\log|x-z|, \beta), -\alpha\right)$, a continuous and bounded function. For any $\epsilon>0$, we have \begin{align}
%     \expect \left[\exp\left\{2N\int f(z) d\mu_N(z)\right\}\right] \leq \exp\left\{2N\left(\int f(z) d\mu(z) + \epsilon\right)\right\} + e^{2N||f||_{\infty}}\mathbb{P}\left(\int f(z) d\mu_N(z) \geq \int f(z)d\mu(z) + \epsilon\right).
% \end{align}
% The entries of $H_N$ are Gaussian and so obey a log Solobev inequality, therefore Theorem 1.5 from  \cite{guionnet2000concentration} gives \begin{align}
%     \mathbb{P}\left(\int f(z) d\mu_N(z) \geq \int f(z)d\mu(z) + \epsilon\right) \lesssim \exp\left\{-\frac{N^2}{8c}\epsilon^2\right\}
% \end{align}
% for some constant $c$ which we need not compute. We have shown \begin{align}
%   \expect|\det(H - xI)| =  A_NB_N \leq \exp\left\{N\left(\int f(z)d\mu(z)\right)\right\} \leq  \exp\left\{N\left(\int \log|x-z|d\mu(z)\right)\right\}.
% \end{align}

% We now need to establish a complimentary lower bound to complete the proof. By Jensen's inequality \begin{align}
%     \expect |\det(H-x)| &\geq \exp\left(N\mathbb{E}\left[\int \log|z-x| d\mu_N(z)\right]\right) \notag\\
%     & \geq \exp\left(N\mathbb{E}\left[\int\max\left(-\alpha,  \log|z-x|\right) d\mu_N(z)\right]\right)  \exp\left(N\expect\left[\int \log|z-x| \indic\{|z-x| \leq e^{-\alpha}\}d\mu_N(z)\right]\right)\notag\\
%     &\geq \exp\left(N\mathbb{E}\left[\int\min\left(\beta, \max\left(-\alpha,  \log|z-x|\right)\right) d\mu_N(z)\right]\right)  \exp\left(N\expect\left[\int \log|z-x| \indic\{|z-x| \leq e^{-\alpha}\}d\mu_N(z)\right]\right)\label{eq:ldp_lower_bound_2_terms}
% \end{align}
% for any $\alpha, \beta >0$. Convergence in law of $\mu_N$ to $\mu$ and the dominated convergence theorem gives \begin{align}
%     \exp\left(N\mathbb{E}\left[\int\min\left(\beta, \max\left(-\alpha,  \log|z-x|\right)\right) d\mu_N(z)\right]\right) \geq \exp\left\{N \left(\int \log|x-z| d\mu(z) + o(1)\right)\right\}
% \end{align}
% for large enough $\beta$, because $\mu$ has compact support. It remains to show that the second term in (\ref{eq:ldp_lower_bound_2_terms})  in the limit $N \rightarrow \infty$. By taking $\alpha\rightarrow\infty$, it is sufficient to show that $\mathbb{E}\mu_N$ is bounded uniformly in $x, x_1, N$. By (\ref{eq:stieljes}), it is sufficient to bound $\langle G_N(z)\rangle$, which is computed via (\ref{eq:lsd_pre_saddle}). Let us define the function $\Phi$ so that \begin{align}
%     \langle G_N(z) \rangle = \frac{2}{b^2} \int d\sigma d\sigma[1] (z-i\sigma_{FF}) e^{-N\Phi(\sigma, \sigma[1])}.
% \end{align}
% Henceforth, $\sigma_{FF}^*, \sigma_{FF}[1]^*, \sigma_{BB}^*, \sigma_{BB}[1]^*$ are the solution to the saddle point equations (\ref{eq:boson_saddle1}-\ref{eq:ferm_saddle2}) and  $\tilde{\sigma}_{FF}, \tilde{\sigma}_{FF}[1], \tilde{\sigma}_{BB}, \tilde{\sigma}_{BB}[1]$ are integration variables in a small region around the saddle point. Around the saddle point \begin{align}
%     z - i\sigma_{FF} = z - i\sigma_{FF}^* - iN^{-\frac{1}{r}}\tilde{\sigma}_{FF}
% \end{align}
% for some $r\geq 2$. We use the notation $\vec{\sigma}$ for $(\sigma_{BB}, \sigma_{BB}[1], \sigma_{FF}, \sigma_{FF}[1])$ and similarly $\vec{\sigma}_B, \vec{\sigma}_F$. While the Hessian of $\Phi$ may not in general vanish at the saddle point, \begin{align}
%     \int d\tilde{\sigma}d\tilde{\sigma}[1] \tilde{\sigma}_{FF} e^{-N \tilde{\vec{\sigma}}^T \nabla^2 \Phi^* \tilde{\vec{\sigma}}} = 0
% \end{align}
% and so we must go to at least the cubic term in the expansion of $\Phi$ around the saddle point, i.e. \begin{align}
%       \langle G_N(z) \rangle = G(z) -  \frac{2i}{b^2 N^{5/3}}\underbrace{\int_{-\infty}^{\infty} d\tilde{\vec{\sigma}}_B d\tilde{\vec{\sigma}}_F \tilde{\sigma}_{FF} e^{-\frac{1}{6} \tilde{\sigma}^i \tilde{\sigma}^j \tilde{\sigma}^k \partial_{ijk}\Phi^*}}_{E(z; x_1)} + \text{ exp. smaller terms}.
% \end{align}
% The bosonic and fermionic coordinates do not interact, so we can consider derivatives of $\Phi$ as block tensors. Simple differentiation gives \begin{align}
%     (\nabla\Phi)_B &= \left(\begin{array}{c}
%         \frac{2}{b^2} - \kappa\left(\sigma_{BB} + \sigma_{BB}[1] + z + x_1\right)^{-2} - \kappa'\left(\sigma_{BB} + z\right)^{-2}  \\
%         \frac{2}{b_1^2} - \left(\sigma_{BB} + \sigma_{BB}[1] + z + x_1\right)^{-2}\end{array}\right)\notag\\
%   \implies  (\nabla^2\Phi)_B &= \left(\begin{array}{cc}
%       2\kappa\left(\sigma_{BB} + \sigma_{BB}[1] + z + x_1\right)^{-3} + 2\kappa'\left(\sigma_{BB} + z\right)^{-3}  &
%       2\kappa\left(\sigma_{BB} + \sigma_{BB}[1] + z + x_1\right)^{-3}\\
%      2\left(\sigma_{BB} + \sigma_{BB}[1] + z + x_1\right)^{-3} &
%       2\left(\sigma_{BB} + \sigma_{BB}[1] + z + x_1\right)^{-3}
%       \end{array}\right)\\
%  \implies (\nabla^3\Phi)_B^* &= \left(\left(\begin{array}{cc}
%       A\kappa + B\kappa' & A\kappa \\
%       A &  A
%  \end{array}\right), A\left(\begin{array}{cc}
%       \kappa & \kappa \\
%       1 &  1
%  \end{array}\right) \right),     
% \end{align}
% where \begin{align}
%     A_B = -\frac{6}{\left(\sigma_{BB}^* + \sigma_{BB}^*[1] + z + x_1\right)^4}, ~~~ B_B= -\frac{6}{\left(\sigma_{BB}^* + z\right)^4}.
% \end{align}

% Let $\xi_1, \xi_2 = \tilde{\sigma}_{BB}, \tilde{\sigma}_{BB}[1]$. Then \begin{align}
%   ( \tilde{\sigma}^i \tilde{\sigma}^j \tilde{\sigma}^k \partial_{ijk}\Phi^*)_B &= \left(A_B\kappa + B_B\kappa'\right)\xi_1^3 + A_B(2\kappa +1 ) \xi_1^2\xi_2[1] + A_B(\kappa +2 ) \xi_1\xi_2^2 + A_B\xi_2^3\notag\\
%   &= A_B\left[\xi_2^3 + (2\kappa +1 )\xi_2\xi_1^2 +(2+ \kappa)\xi_1\xi_2^2 + C\xi_1^3\right] + \left(B_B\kappa' + A_B\kappa - CA_B\right)\xi_1^3
% \end{align}
% for any $C$. Let $\xi_1 = a_1\xi_1'$ and then choose $C = a_1^{-3}$ and $a_1 = (2+\kappa)(2\kappa + 1)^{-1}$ to give \begin{align}
%      ( \tilde{\sigma}^i \tilde{\sigma}^j \tilde{\sigma}^k \partial_{ijk}\Phi^*)_B &= A_B(\xi_1' + \xi_2)^3 + (B_B\kappa' + A_B\kappa - CA_B)a_1^3(\xi_1')^3 \equiv A_B\eta^3 + D_B\xi^3
% \end{align}
% with $\eta = \xi_1' + \xi_2$, $\xi=\xi_1'$, $D_B=B_B\kappa' + A_B\kappa - a_1^{-3}A_B$. The expressions for $ ( \tilde{\sigma}^i \tilde{\sigma}^j \tilde{\sigma}^k \partial_{ijk}\Phi^*)_F$ follow identically. We thus have \begin{align}
%     E(z;x_1) \propto \left(\int_0^{\infty} d\xi ~ \xi \int_{\xi}^{\infty}d\eta ~ e^{A_F\eta^3 + D_F\xi^3}\right)\left(\int_0^{\infty} d\xi ~  \int_{\xi}^{\infty}d\eta ~ e^{A_B\eta^3 + D_B\xi^3}\right)
% \end{align} 
% or perhaps with the the integration ranges reversed depending on the signs of $\Re A_F, \Re A_B, \Re D_F, \Re D_B$. We have \begin{align}
%     |E(z;  x_1)| & \leq  \left|\int_0^{\infty} d\xi ~ \xi \int_{\xi}^{\infty}d\eta ~ e^{A_F\eta^3 + D_F\xi^3}\right|\cdot\left|\int_0^{\infty} d\xi ~  \int_{\xi}^{\infty}d\eta ~ e^{A_B\eta^3 + D_B\xi^3}\right|\notag\\
%     & \leq  \int_0^{\infty} d\xi ~ \xi \int_{\xi}^{\infty}d\eta ~| e^{A_F\eta^3 + D_F\xi^3}|\cdot\int_0^{\infty} d\xi ~  \int_{\xi}^{\infty}d\eta ~| e^{A_B\eta^3 + D_B\xi^3}|\notag\\
%     & \leq  \int_0^{\infty} d\xi ~ \xi \int_{0}^{\infty}d\eta ~| e^{A_F\eta^3 + D_F\xi^3}|\cdot\int_0^{\infty} d\xi ~  \int_{0}^{\infty}d\eta ~| e^{A_B\eta^3 + D_B\xi^3}|\notag\\
%     & \leq \left(|\mathfrak{M} D_F|\right)^{-2/3}\left(|\mathfrak{M} A_F|\right)^{-1/3}
%     \left(|\mathfrak{M} D_B|\right)^{-1/3}
%     \left(|\mathfrak{M} A_B|\right)^{-1/3}\left(\int_0^{\infty} e^{-\xi^3}d\xi\right)^3 \left(\int_0^{\infty}~ \xi e^{-\xi^3}d\xi\right)\label{eq:esd_error_bound}
% \end{align}
% where we have defined \begin{align}
%     \mathfrak{M} y = \begin{cases} \Re y ~~ &\text{if } \Re y \neq 0, \\
%     \Im y ~~ &\text{if } \Re y = 0. \\
%     \end{cases}
% \end{align}
% This last bound follows from a standard Cauchy rotation of integration contour if any of $D_F, A_F, D_B, A_B$ has vanishing real part.
% (\ref{eq:esd_error_bound}) is valid for $D_B, A_B, D_F, A_F \neq 0$, but if $D_B=0$ and $A_B\neq 0$, then the preceeding calculations are simplified and we still obtain an upper bound but proportional to $(|\mathfrak{M} A_B|)^{-1/3}$. Similarly with $A_B=0$ and $D_B\neq 0$ and similarly $A_F, D_F$. The only remaining cases are $A_B = D_B =0$ or $A_F = D_F =0$. Referring to definitions of $A_B, D_B, A_F, D_F$ and the saddle point equations (\ref{eq:boson_saddle1}-\ref{eq:ferm_saddle2}), these cases correspond precisely to  $\sigma_{FF}^* =0$. Recalling (\ref{eq:master_quartic}), one can easily show that $\sigma_{FF}^* =0$ if an only if \begin{align}
%     z = \frac{-x_1 \pm \sqrtsign{x_1^2 + 4\kappa^{-1}\kappa' b_1^2 ( 1 - \frac{\kappa}{\kappa'})}}{2}\label{eq:null_set}.
% \end{align}
% For small $\epsilon>0$, let $U=\left\{ (z, x_1)\in\mathbb{R}^2 \mid (\ref{eq:null_set}) \text{ holds}\right\}$ and  \begin{align}
%     U_{\epsilon} = \bigcup_{(z, x_1)\in U} B_{\epsilon}((z, x_1)).
% \end{align} We have shown that for all $(z, x_1)\in\mathbb{R}^2/ U_{\epsilon}$, there exist constants $c_F, c_B$ (dependent on $\epsilon$) such that \begin{align}
%     |E(z; x_1)| \leq c_F c_B \left(\int_0^{\infty} e^{-\xi^3}d\xi\right)^3 \left(\int_0^{\infty}~ \xi e^{-\xi^3}d\xi\right) \end{align} meaning that $\langle G_N(z)\rangle$ is uniformly bounded in $z, x_1$ in $\mathbb{R}^2/U_{\epsilon}$. Overall, we now have \begin{align}
% &\int_{B/U_{\epsilon}} dx dx_1 ~ \exp\left\{-N\left(\frac{x^2}{2s^2} + \frac{x_1^2}{2s_1^2} - \int \log|z - x| d\mu(z)\right)\right\} \notag\\ + &\int_{U_{\epsilon}} dx dx_1 ~ \exp\left\{-N\left(\frac{x^2}{2s^2} + \frac{x_1^2}{2s_1^2}\right)\right\}\expect|\det(H_N-xI)| + o(1) \notag\\
% \leq &\int_{B} dx dx_1 ~ \exp\left\{-N\left(\frac{x^2}{2s^2} + \frac{x_1^2}{2s_1^2}\right)\right\}\expect|\det(H_N-xI)|\notag\\
% \leq &(1 + o(1))\int_{B} dx dx_1 ~ \exp\left\{-N\left(\frac{x^2}{2s^2} + \frac{x_1^2}{2s_1^2} - \int \log|z - x| d\mu(z)\right)\right\} .
%     \end{align}
%     Taking $\epsilon\rightarrow 0$ completes the proof.
% \end{proof}



\begin{comment}
 \section{Supersymmetric approach - old}
 \subsection{Hybrid method}
 One approach is that described in \cite{nock2017characteristic} and used in \cite{baskerville2020loss}. Refering to \cite{baskerville2020loss}, (5.14) therein is modified here to\footnote{Note that we are being perhaps a little fast-and-loose with the ordering of the even and odd infinitesimals in our supersymmetric algebra - it's right up to a sign.} \begin{align}
     \Delta_{\epsilon} = K_N^{(1)} \prod_{t=1}^2\int d\vec{x}_1[t]d\vec{x}_2[t] d\zeta_1[t]d \zeta_1^*[t]d\zeta_2[t] d\zeta_2^*[t]\exp\Bigg\{& -i b_1\sqrtsign{2N} \Tr M_1A - ib_2\sqrtsign{2\kappa N}\Tr M_2 A[1]\notag \\ 
     & + i(x_1 + i\epsilon)\Tr A + ix_2 \Tr A[1]\Bigg\}\notag \\
     \implies  \mathbb{E}_{M_1, M_2}\Delta_{\epsilon} = K_N^{(1)} \prod_{t=1}^2\int d\vec{x}_1[t]d\vec{x}_2[t] d\zeta_1[t]d \zeta_1^*[t]d\zeta_2[t] d\zeta_2^*[t]\exp\Bigg\{& - \frac{b_1^2}{4N^2}\Tr (A+A^T)^2 - \frac{b_2^2}{4\kappa N}\Tr (A[1]+A[1]^T)^2 \notag \\ &+ i(x_1 + i\epsilon)\Tr A + ix_2 \Tr A[1]\Bigg\}
 \end{align}
 where here we split the $N$ dimensional commuting and anti-commuting vectors as $\vec{x} = (\vec{x}[1], \vec{x}[2])$ etc for $\kappa N$-dimensional $\vec{x}[1]$ and $(1-\kappa)N$-dimensional $\vec{x}[2]$. The matrix $N\times N$ $A$ is given by \begin{align}
     A = \vec{x}_1\vec{x}_1^T + \vec{x}_2\vec{x}_2^T + \zeta_1\zeta_1^{\dagger} + \zeta_2\zeta_2^{\dagger}
 \end{align}
 and the the smaller matrices $A[1], A[2]$ are defined in the obvious way. We then can proceed as in \cite{baskerville2020loss} and we introduce matrices \begin{align}
     Q_B = \left(\begin{array}{cc} \vec{x}_1^T\vec{x}_1 & \vec{x}_1^\vec{x}_2 \\
     \vec{x}_2^T\vec{x}_1 & \vec{x}_2^T\vec{x}_2\end{array}\right)
 \end{align}
 \begin{align}
     Q_F = \left(\begin{array}{cc} \zeta_1^{\dagger}\zeta_1 & \zeta_1^{\dagger}\zeta_2 \\
    \zeta_2^{\dagger}\zeta_1 &\zeta_2^{\dagger}\zeta_2\end{array}\right)
 \end{align}
 for which we have the convenient facts \begin{align}
     Q_B &= Q_B[1] + Q_B[2]\\
     Q_F &= Q_F[1] + Q_F[2].
 \end{align}
 Following the procedure in \cite{baskerville2020loss} but without the approximations introduced there to cope with the low-rank matrix $S$, we can reduce to integrals over only the matrices $Q_B[t], Q_F[t]$ for $t=1,2$ and a few extra variables. We then ultimately diagonalise to arrive at an expression analogous to (5.61) in \cite{baskerville2020loss}. We end up with exponential terms in 8 variables: $p_1[t], p_2[t], r_1[t], r_2[t]$ for $t=1,2$, as one would eexpect. The $p$ and $r$ variables are un-coupled, and we obtain roughly the same functions $\psi$ as in \cite{baskerville2020loss} in the form $$\psi(p_1[1]) + \psi(p_1[2]) + \psi(p_2[1]) + \psi(p_2[2]).$$ There is, however, a coupling term of the form \begin{align}
     p_1[1]p_1[2] + p_2[1]p_2[2] + p_1[1]p_2[2] + p_1[2]p_1[1]
 \end{align}
 and so the saddle point equations are 4 coupled quadratics in the $p$ variables and similar for $r$. The equations do not appear to be reducible. Mathematica produces very complicated expressions.
 
 \subsection{Sigma representation approach}
 \cite{guhr1990isospin} approaches a similar problem, namely that of the correlation functions of $H = H_U + \alpha H_C$ where $H_U$ is a block diagonal matrix of with $N\times N$ i.i.d. GUEs on the diagonal blocks and where $H_C$ is an off-diagonal block matrix with an identical $N\times N$ complex Ginibre on the off-diagonals. Following the approach used in \cite{guhr1990isospin}, we introduce supersymmetric variables as above, but we use \begin{align}
     \frac{1}{4}\Tr (A+A^T)^2 = \trg Q^2
 \end{align}
 where $Q$ is the $6\times 6$ matrix $Q = B^{\dagger}B$ where $B = (\vec{x}_1, \vec{x}_2, \zeta_1, \zeta_1^*, \zeta_2, \zeta_2^*)$ and $\trg$ is the graded (supersymmetric trace) \cite{efetov_1996}.  We can use the `super Fourier transform' result \cite{guhr1991dyson} \begin{align}
     \int d[\sigma] e^{-2\trg\sigma^2} e^{-i \trg \sigma Q} \propto e^{-\trg Q^2}
 \end{align} where the $6\times 6$ matrix supermatrix $\sigma$ has the same structure as $Q$ but with an opportune factor of $i$ introduced in the Fermion-Fermion block for the sake of convergence. We introduce $\sigma$ and $\sigma[1]$. The approach in  \cite{guhr1990isospin} is then to diagonalise the $\sigma$ supermatrices using various results from \cite{guhr1991dyson}, giving diagonal matrices $S, S[1]$ etc. In that case, because it is the GUE, a nice determinantial form is reached (see (4.44) in \cite{guhr1990isospin}) but I don't believe this difference is going to be important for the order-of-magnitude asymptotics. \cite{guhr1990isospin} then deals with the eigenvalue integrals $S[t]$, $S$ in turn which we can do also for $S[1]$ and $S$, \emph{however} there is a factor of $N$ difference between us and \cite{guhr1990isospin} which allows them to do the following \begin{enumerate}
     \item find saddle points in the $S[t]$ eigenvalues (in terms of $S$)
     \item evaluate at the saddle point
     \item approximate the result to leading order in $N$ (inside the exponent)
     \item do saddle point analysis in the $S$ eigenvalues for some cases.
 \end{enumerate}
 We cannot do step C owing to the factor of $N$ discrepancy. This factor of $N$ discrepancy seems to be  due to normalisation of the G\{U/O\}E matrices, namely we have (along with \cite{baskerville2020loss, nock2017characteristic}) \begin{align}
     P_{GOE}(M) \propto e^{-\frac{N}{2} \Tr M^2}
 \end{align}
 whereas \cite{guhr1991dyson, guhr1990isospin} has (see (2.1) in \cite{guhr1991dyson})
 \begin{align}
     P_{GUE}(M) \propto e^{-\frac{1}{2} \Tr M^2}.
 \end{align}
 This distinction seems trivial but I am suspecting that it's important and relates to the distinction between studying local correlation functions in the limit (as in \cite{guhr1990isospin}) and macroscopic properties as in \cite{baskerville2020loss}?\\
 
 Continuing without the step C above, we end up with integration over 12 variables: $s_1[1],\ldots s_6[1]$ and $s_1, \ldots, s_6$. The saddle point equations are again very similar to \cite{baskerville2020loss} but we get coupled quaratics in $(s_i, s_i[1])$ for each $i$, but no coupling between $i$ values. This seems more tractable than the previous subsection, but the equations are not reducible and so the saddle points are still going to contain nested radicals. It may be possible to proceed from here, but we will have to be \emph{very} careful with choices of branch and it will certainly be a mess, but may just be tractable with a bit of numerics.
 
 
 \subsubsection{Expansion in small variance}
 
We introduced the variance ratio parameter $\sigma_z$ into our model. We will be interested in critical behaviour relating to this parameter (along with $\kappa, p, q$). We can  solve the saddle point equaitons for the $S, S[1]$ eigenvalues to leading order in $\sigma_z$. The equations predictably de-couple and the result is that the order-of-magnitude function $\Theta$ is just a sum of the functions for each of the spin glasses independently. Note that, as we are interested in the \emph{sign} of $\Theta$, there is still non-trivial behaviour resulting from simply summing the $\Theta$ function from each spin glass.\footnote{N.B. the results should not consistently return that of a single spin glass when $\sigma_z = 0$ because the Hessian in the Kac-Rice determinant is then singular.} 
\end{comment}




% \begin{align}
%   \expect \left[\exp\left\{2e^{-\beta/2} \Tr |H_N- xI|\right\}\right]   &= \left(\int dh ~ e^{-\frac{N}{2(b^2+b_1^2)}h^2} e^{2e^{-\beta/2}|h- x -x_1|}\right)^{\kappa N} \left(\int dh ~ e^{-\frac{N}{2(b^2)}h^2} e^{2e^{-\beta/2}|h- x |}\right)^{\kappa' N}\notag\\
%   &\leq \left(e^{-2e^{-\beta/2}(|x| + |x_1|)}e^{\frac{2(b^2 + b_1^2)}{N} e^{-\beta}} \right)^{\kappa N} \left(e^{-2e^{-\beta/2}|x|}e^{\frac{2b^2}{N} e^{-\beta}} \right)^{\kappa' N}\notag\\
%   &= \exp\left\{-2e^{-\beta/2} N (|x|  +\kappa|x_1|)\right\}\exp\left\{2e^{-\beta}\left(b^2 + \kappa b_1^2\right)\right\}\notag\\
%   & \leq \exp\left\{2e^{-\beta}\left(b^2 + \kappa b_1^2\right)\right\}\notag\\
%   &\rightarrow 1 
% \end{align}
% uniformly in $N$ as $\beta\rightarrow\infty$.

% \begin{align}
%     \expect \left[\exp\left\{2e^{-\frac{\beta}{2}} \Tr |H_N- xI|\right\}\right]   &\leq  \prod_{1\leq i\leq j \leq N}    \expect_{h_{ij}\sim \mathcal{N}(0,\frac{1}{N}(b^2 + b_1^2))}  \exp\left\{ 4e^{-
%     \frac{\beta}{2}}\left( |x| + |x_1| + |h_{ij}|\right)\right\}\notag\\
%     &\leq \exp\left\{2(N+1)^2e^{-\frac{\beta}{2}}(|x| + |x_1|)\right\} \left(\int \frac{dh}{Z_N} ~ e^{-\frac{Nh^2}{2(b^2 + b_1^2)}} e^{4e^{-\beta/2}|h|}\right)^{\frac{1}{2}(N+1)^2}\notag\\
%     &\leq \exp\left\{2(N+1)^2e^{-\frac{\beta}{2}}(|x| + |x_1|)\right\} \left(\int \frac{dh}{2Z_N} ~ \left[e^{-\frac{Nh^2}{2(b^2 + b_1^2)}} e^{4e^{-\frac{\beta}{2}}h} + e^{-\frac{Nh^2}{2(b^2 + b_1^2)}} e^{-4e^{-\frac{\beta}{2}}h}\right]\right)^{\frac{1}{2}(N+1)^2}\notag\\
%     &=\exp\left\{2(N+1)^2e^{-\frac{\beta}{2}}(|x| + |x_1|)\right\} \left(\frac{1}{2}\left[e^{\frac{8e^{-\beta}(b^2 + b_1^2)}{N}} +e^{-\frac{8e^{-\beta}(b^2 + b_1^2)}{N}}\right]  \right)^{\frac{1}{2}(N+1)^2}\notag\\
%     &\leq \exp\left\{2(N+1)^2e^{-\frac{\beta}{2}}(|x| + |x_1|)\right\} \left(e^{\frac{8e^{-\beta}(b^2 + b_1^2)}{N}}\right)^{\frac{1}{2}(N+1)^2}\notag\\
%     &= \exp\left\{2(N+1)^2e^{-\frac{\beta}{2}}(|x| + |x_1|)\right\} \exp\left\{e^{-\beta}\mathcal{O}(N)\right\}\notag\\
%     &\rightarrow 1
% \end{align}
